USRP-Based Single Anchor Positioning: AoA with 5G Uplink Signals, and UWB Ranging

This paper presents a novel testbed designed for 5th-Generation (5G) positioning using Universal Software Radio Peripherals (USRPs). The testbed integrates multiple units: an Operation Unit for test management, a User Unit equipped with an Ettus E312 USRP, and a Station Unit featuring an Ettus N310 USRP equipped with a three-element Uniform Linear Array for Angle of Arrival estimation. Alongside ultra wideband ranging, the testbed estimates the user's position relative to the base station. Signal processing algorithms are executed in a dedicated processing unit. Key challenges addressed include phase misalignment between RX channel pairs due to different Local Oscillators in the Ettus N310, necessitating real-time calibration for precise signal alignment. High sampling rates (up to 61.44 MSps) result in large IQ sample files, managed efficiently using a snapshot technique to optimize storage without compromising testbed positioning capabilities. The testbed synchronizes angular measurements with ranging estimates allowing consistent performance evaluation for real-life cases of dynamic users (e.g. pedestrian). Experimental results demonstrate the testbed's effectiveness in achieving accurate pedestrian user localization.

==> 05XX/0510/Data/cdf_vld_test_0510_SID2_F2p451GHz_TxG89_RxG75_TD300s_SL9ms.tex <==
0	0.101971	
0.004	0.101971	
0.008	0.186688	
0.012	0.19812	
0.016	0.204955	
0.02	0.236696	
0.024	0.278597	
0.028	0.320029	
0.032	0.328177	
0.036	0.329442	
0.04	0.348548	
0.044	0.374163	
0.048	0.396639	
0.052	0.417857	
0.056	0.437534	
0.06	0.438288	
0.064	0.461877	
0.068	0.471591	
0.072	0.508981	
0.076	0.530323	
0.08	0.537513	
0.084	0.558171	
0.088	0.559192	
0.092	0.567924	
0.096	0.573716	
0.1	0.577487	
0.104	0.586069	
0.108	0.646226	
0.112	0.688609	
0.116	0.694873	
0.12	0.732838	
0.124	0.736537	
0.128	0.74439	
0.132	0.74963	
0.136	0.782885	
0.14	0.786312	
0.144	0.801134	
0.148	0.810068	
0.152	0.817297	
0.156	0.82248	
0.16	0.858186	
0.164	0.862841	
0.168	0.878641	
0.172	0.885711	
0.176	0.936939	
0.18	0.949006	
0.184	0.955549	
0.188	0.981311	
0.192	0.986754	
0.196	0.987783	
0.2	0.995063	
0.204	1.00824	
0.208	1.01466	
0.212	1.02357	
0.216	1.02698	
0.22	1.02938	
0.224	1.04342	
0.228	1.05323	
0.232	1.05468	
0.236	1.06692	
0.24	1.07474	
0.244	1.08663	
0.248	1.08924	
0.252	1.09628	
0.256	1.10662	
0.26	1.13585	
0.264	1.13639	
0.268	1.14621	
0.272	1.14747	
0.276	1.14824	
0.28	1.15109	
0.284	1.16389	
0.288	1.16534	
0.292	1.20539	
0.296	1.21508	
0.3	1.28845	
0.304	1.29243	
0.308	1.31623	
0.312	1.33427	
0.316	1.342	
0.32	1.38117	
0.324	1.38759	
0.328	1.42624	
0.332	1.45848	
0.336	1.49108	
0.34	1.57254	
0.344	1.58839	
0.348	1.60958	
0.352	1.67763	
0.356	1.73369	
0.36	1.73531	
0.364	1.75115	
0.368	1.76481	
0.372	1.77333	
0.376	1.79728	
0.38	1.83021	
0.384	1.83415	
0.388	1.85508	
0.392	1.86322	
0.396	1.88717	
0.4	1.89985	
0.404	1.93689	
0.408	1.93887	
0.412	1.97013	
0.416	2.09371	
0.42	2.10042	
0.424	2.11404	
0.428	2.1344	
0.432	2.13909	
0.436	2.14682	
0.44	2.22713	
0.444	2.2739	
0.448	2.27442	
0.452	2.40672	
0.456	2.43507	
0.46	2.45159	
0.464	2.48205	
0.468	2.4836	
0.472	2.54233	
0.476	2.54693	
0.48	2.5621	
0.484	2.58323	
0.488	2.61809	
0.492	2.67455	
0.496	2.70209	
0.5	2.72264	
0.504	2.77001	
0.508	2.7759	
0.512	2.7923	
0.516	2.81004	
0.52	2.90178	
0.524	2.95765	
0.528	3.01464	
0.532	3.21853	
0.536	3.24232	
0.54	3.26859	
0.544	3.30008	
0.548	3.37603	
0.552	3.45013	
0.556	3.4532	
0.56	3.48008	
0.564	3.5559	
0.568	3.60453	
0.572	3.60956	
0.576	3.7393	
0.58	3.90773	
0.584	3.92346	
0.588	3.9576	
0.592	3.96431	
0.596	3.96472	
0.6	3.98435	
0.604	4.06129	
0.608	4.13676	
0.612	4.17078	
0.616	4.17315	
0.62	4.17617	
0.624	4.24032	
0.628	4.46312	
0.632	4.55828	
0.636	4.77059	
0.64	4.784	
0.644	4.81625	
0.648	4.87012	
0.652	4.91363	
0.656	4.94632	
0.66	4.97364	
0.664	5.00719	
0.668	5.20096	
0.672	5.24762	
0.676	5.39488	
0.68	5.51455	
0.684	5.6157	
0.688	5.71124	
0.692	5.93415	
0.696	5.97491	
0.7	6.08976	
0.704	6.20234	
0.708	6.29642	
0.712	6.36015	
0.716	6.38263	
0.72	6.38316	
0.724	6.42358	
0.728	6.47216	
0.732	6.50886	
0.736	6.66359	
0.74	6.75693	
0.744	6.78061	
0.748	6.90669	
0.752	7.10369	
0.756	7.1284	
0.76	7.16248	
0.764	7.19977	
0.768	7.39284	
0.772	7.54692	
0.776	7.58385	
0.78	7.67056	
0.784	7.73619	
0.788	7.7389	
0.792	7.83074	
0.796	7.84766	
0.8	7.88361	
0.804	7.88452	
0.808	7.95886	
0.812	8.02039	
0.816	8.15987	
0.82	8.2062	
0.824	8.28693	
0.828	8.3104	
0.832	8.44934	
0.836	8.46956	
0.84	8.69612	
0.844	8.75655	
0.848	8.82398	
0.852	8.95237	
0.856	9.03407	
0.86	9.03696	
0.864	9.20758	
0.868	9.21622	
0.872	9.2852	
0.876	9.89734	
0.88	10.5256	
0.884	10.5907	
0.888	10.6117	
0.892	10.838	
0.896	10.8846	
0.9	11.1147	
0.904	11.162	
0.908	11.208	
0.912	12.2623	
0.916	13.0875	
0.92	13.1397	
0.924	13.2853	
0.928	13.6381	
0.932	13.6406	
0.936	13.6437	
0.94	13.734	
0.944	13.791	
0.948	13.8592	
0.952	14.098	
0.956	14.2846	
0.96	14.5942	
0.964	14.8297	
0.968	15.0942	
0.972	15.3517	
0.976	15.6277	
0.98	15.7771	
0.984	16.0954	
0.988	16.2911	
0.992	16.5569	
0.996	17.8114	
1	18.387	


==> 05XX/0510/Data/pdf_vld_test_0510_SID2_F2p451GHz_TxG89_RxG75_TD300s_SL9ms.tex <==
0.00176495	0.0188157	
0.202473	0.212516	
0.266691	0.406216	
0.277578	0.599917	
0.263393	0.793617	
0.239252	0.987317	
0.213468	1.18102	
0.189686	1.37472	
0.169053	1.56842	
0.151603	1.76212	
0.136964	1.95582	
0.124676	2.14952	
0.114313	2.34322	
0.105515	2.53692	
0.0979913	2.73062	
0.0915135	2.92432	
0.0858998	3.11802	
0.0810058	3.31172	
0.0767156	3.50542	
0.0729351	3.69912	
0.0695872	3.89282	
0.0666074	4.08652	
0.063942	4.28022	
0.0615451	4.47392	
0.0593775	4.66762	
0.0574057	4.86132	
0.0556006	5.05502	
0.0539372	5.24872	
0.0523936	5.44242	
0.0509511	5.63613	
0.0495934	5.82983	
0.0483064	6.02353	
0.0470781	6.21723	
0.0458983	6.41093	
0.0447584	6.60463	
0.043651	6.79833	
0.0425704	6.99203	
0.0415116	7.18573	
0.040471	7.37943	
0.0394458	7.57313	
0.0384338	7.76683	
0.0374339	7.96053	
0.0364453	8.15423	
0.0354681	8.34793	
0.0345026	8.54163	
0.0335497	8.73533	
0.0326105	8.92903	
0.0316865	9.12273	
0.0307795	9.31643	
0.0298913	9.51013	
0.0290238	9.70383	
0.0281794	9.89753	
0.0273599	10.0912	
0.0265677	10.2849	
0.0258046	10.4786	
0.0250727	10.6723	
0.0243738	10.866	
0.0237095	11.0597	
0.0230812	11.2534	
0.0224901	11.4471	
0.0219369	11.6408	
0.0214223	11.8345	
0.0209463	12.0282	
0.0205086	12.2219	
0.0201087	12.4156	
0.0197452	12.6093	
0.0194165	12.803	
0.0191205	12.9967	
0.0188542	13.1904	
0.0186144	13.3841	
0.0183971	13.5778	
0.0181978	13.7715	
0.0180112	13.9652	
0.0178317	14.1589	
0.0176527	14.3526	
0.0174674	14.5463	
0.0172683	14.74	
0.0170476	14.9337	
0.0167972	15.1274	
0.0165087	15.3211	
0.016174	15.5148	
0.0157851	15.7085	
0.015335	15.9022	
0.0148178	16.0959	
0.0142296	16.2896	
0.0135691	16.4833	
0.012839	16.677	
0.0120467	16.8707	
0.0112063	17.0644	
0.0103393	17.2581	
0.00947563	17.4518	
0.00865229	17.6455	
0.00790858	17.8392	
0.00727295	18.0329	
0.00673599	18.2266	
0.00620282	18.4203	
0.00543269	18.614	
0.00404529	18.8077	
0.00189889	19.0014	
0.000174704	19.1951	


==> 05XX/0510/Data/vld_test_0510_SID2_F2p451GHz_TxG89_RxG75_TD300s_SL9ms.tex <==
1	0.719552	15.3281	38.2878	21.7884	0	8784.18	2.10385	35.1246	35.1775	34.9692	-15.3178	-0.562709	-15	0	15	-0	0.328086	2.10385	NaN	NaN	
2	0.0182188	15.3515	38.2878	21.7884	0	8785.18	3.04077	35.2812	35.1829	35.1537	-15.3299	-0.814347	-15	0	15	-0	0.351538	3.04077	NaN	NaN	
3	-0.0334479	15.3703	38.2878	21.7884	0	8786.18	3.45603	35.2911	35.1886	35.1702	-15.3423	-0.926561	-15	0	15	-0	0.370299	3.45603	NaN	NaN	
4	0.0259965	15.3773	38.2878	21.7884	0	8787.18	1.40585	35.259	35.1466	35.3109	-15.3727	-0.37727	-15	0	15	-0	0.377335	1.40585	NaN	NaN	
5	-0.291618	15.3398	38.2878	21.7884	0	8788.18	2.67862	35.3309	35.115	35.3094	-15.3231	-0.716886	-15	0	15	-0	0.339812	2.67862	NaN	NaN	
6	-0.0149934	15.3398	38.2878	21.7884	0	8789.18	2.26239	35.2601	35.1539	35.1783	-15.3279	-0.605552	-15	0	15	-0	0.339813	2.26239	NaN	NaN	
7	-0.00456632	15.3328	38.2878	21.7884	0	8790.18	1.69309	35.2156	34.7011	35.1343	-15.3261	-0.453017	-15	0	15	-0	0.332776	1.69309	NaN	NaN	
8	-0.480059	15.3328	38.2878	21.7884	0	8791.18	3.68086	35.3037	35.1939	35.1549	-15.3011	-0.984348	-15	0	15	-0	0.332776	3.68086	NaN	NaN	
9	-0.408068	15.3164	38.2878	21.7884	0	8792.18	-0.347437	35.239	34.9035	35.2528	-15.3161	0.0928767	-15	0	15	-0	0.316361	0.347437	NaN	NaN	
10	-0.274501	15.3281	38.2878	21.7884	0	8793.18	1.83509	35.1642	34.7422	35.1154	-15.3202	-0.490849	-15	0	15	-0	0.328087	1.83509	NaN	NaN	
11	-0.214142	15.3422	38.2878	21.7884	0	8794.18	0.571877	35.0975	34.6213	35.1094	-15.3414	-0.15313	-15	0	15	-0	0.342157	0.571877	NaN	NaN	
12	-0.245683	15.314	38.2878	21.7884	0	8795.18	2.87403	35.1483	35.0458	35.1386	-15.2948	-0.76785	-15	0	15	-0	0.314016	2.87403	NaN	NaN	
13	-0.711281	15.3375	38.2878	21.7884	0	8796.18	3.30216	35.1148	35.0314	35.1401	-15.312	-0.883465	-15	0	15	-0	0.337467	3.30216	NaN	NaN	
14	0.0623097	15.3093	38.2878	21.7884	0	8797.18	2.86057	35.1381	35.0508	35.1075	-15.2902	-0.764022	-15	0	15	-0	0.309325	2.86057	NaN	NaN	
15	-0.246496	15.3328	38.2878	21.7884	0	8798.18	3.10147	35.1441	35.0039	35.0503	-15.3103	-0.82957	-15	0	15	-0	0.332776	3.10147	0.0187502	1.0147	
16	-0.348031	15.3187	38.2878	21.7884	0	8799.18	2.51002	35.1376	35.0509	35.1123	-15.304	-0.67087	-15	0	15	-0	0.318706	2.51002	0.0192138	1.01315	
17	-0.167892	15.6119	38.2878	21.7884	0	8800.18	4.44057	35.1611	35.1258	35.2449	-15.565	-1.20875	-15	0	15	-0	0.611853	4.44057	0.0738684	1.13591	
18	0.258219	15.5767	38.2878	21.7884	0	8801.18	3.00167	35.2057	35.1291	35.1129	-15.5553	-0.815672	-15	0	15	-0	0.576675	3.00167	0.0937504	1.11352	
19	-0.164851	15.4711	38.2878	21.7884	0	8802.18	3.93595	35.2784	35.1779	35.3543	-15.4347	-1.06196	-15	0	15	-0	0.471142	3.93595	0.0975186	1.13742	
20	0.436944	15.4453	38.2878	21.7884	0	8803.18	3.73171	35.2716	35.2	35.2396	-15.4126	-1.00525	-15	0	15	-0	0.445346	3.73171	0.0987078	1.1741	
21	-0.275184	15.2906	38.2878	21.7884	0	8804.18	3.05534	35.2498	35.1771	35.2163	-15.2688	-0.814993	-15	0	15	-0	0.290563	3.05534	0.100956	1.17197	
22	-0.155115	15.3281	38.2878	21.7884	0	8805.18	2.68617	35.2801	35.1734	35.2241	-15.3112	-0.718356	-15	0	15	-0	0.328086	2.68617	0.101111	1.13677	
23	-0.201977	15.504	38.2878	21.7884	0	8806.18	3.28134	35.2875	35.1876	35.2545	-15.4786	-0.887431	-15	0	15	-0	0.503974	3.28134	0.105334	1.11909	
24	0.702038	15.3539	38.2878	21.7883	0	8807.18	4.6787	35.2625	34.8604	35.2107	-15.3027	-1.25238	-15	0	15	-0	0.353883	4.6787	0.103936	1.00232	
25	0.396763	15.3328	38.2878	21.7883	0	8808.18	5.49339	35.2203	34.5971	35.2345	-15.2624	-1.46782	-15	0	15	-0	0.332777	5.49339	0.10374	1.12155	
26	0.152253	15.3304	38.2878	21.7883	0	8809.18	4.10687	35.2361	34.6136	35.2135	-15.2911	-1.09792	-15	0	15	-0	0.330431	4.10687	0.10418	0.844041	
27	0.844231	15.2859	38.2878	21.7883	0	8810.18	4.86295	35.2451	33.9572	35.2184	-15.2308	-1.29582	-15	0	15	-0	0.285873	4.86295	0.105894	0.887503	
28	0.616249	15.3046	38.2878	21.7883	0	8811.18	4.75099	35.2318	34.8414	35.2232	-15.252	-1.26761	-15	0	15	-0	0.304635	4.75099	0.107356	0.922758	
29	0.761611	15.3445	38.2878	21.7883	0	8812.18	3.76529	35.2351	34.4142	35.0257	-15.3114	-1.00767	-15	0	15	-0	0.344503	3.76529	0.105926	0.888235	
30	-0.0326327	15.3891	38.2878	21.7883	0	8813.18	2.64123	35.2164	33.6706	35.252	-15.3727	-0.709155	-15	0	15	-0	0.389061	2.64123	0.104793	0.922374	
31	0.263052	15.307	38.2878	21.7883	0	8814.18	1.83276	35.2022	34.1234	35.2497	-15.2991	-0.489551	-15	0	15	-0	0.30698	1.83276	0.105425	1.00289	
32	0.374128	15.518	38.2878	21.7883	0	8815.18	3.29082	34.9483	32.7313	34.9158	-15.4925	-0.890798	-16.0938	-0	16.0938	-0	0.575705	3.29082	0.100323	0.99028	
33	0.973802	16.1466	38.2878	21.7883	0	8816.18	3.12257	35.2963	35.076	35.2986	-16.1226	-0.879536	-17.1875	-0	17.1875	-0	1.04095	3.12257	0.191994	0.984891	
34	0.0121885	17.1081	38.2878	21.7883	0	8817.18	2.40086	35.1773	35.0785	35.2447	-17.0931	-0.716669	-18.2812	-0	18.2812	-0	1.17317	2.40086	0.273534	1.03514	
35	0.314885	18.0321	38.2878	21.7883	0	8818.18	3.95987	35.1395	33.9933	35.2119	-17.989	-1.24526	-19.375	-0	19.375	-0	1.34292	3.95987	0.354607	1.03919	
36	0.183052	19.1601	38.2878	21.7883	0	8819.18	11.4932	35.1674	34.5816	35.2257	-18.7759	-3.81768	-20.4688	-0	20.4688	-0	1.30864	11.4932	0.40059	2.27499	
37	-0.0939368	20.124	38.2878	21.7883	0	8820.18	2.85259	35.2661	35.0476	35.1819	-20.099	-1.0015	-21.5625	-0	21.5625	-0	1.43852	2.85259	0.447628	2.26769	
38	1.03169	21.1629	38.2878	21.7883	0	8821.18	2.3932	35.0921	34.8468	35.0385	-21.1444	-0.883701	-22.6562	-0	22.6562	-0	1.49336	2.3932	0.492274	2.30383	
39	0.498104	22.1901	38.2878	21.7883	0	8822.18	2.65103	30.0732	27.6775	29.8434	-22.1663	-1.02635	-23.75	-0	23.75	-0	1.55992	2.65103	0.523144	2.32742	
40	0.344961	23.365	38.2878	21.7883	0	8823.18	4.93299	31.1266	30.9328	31.415	-23.2785	-2.00917	-24.8438	-0	24.8438	-0	1.47874	4.93299	0.531279	2.3057	
41	-0.0669128	24.547	38.2878	21.7882	0	8824.18	1.84088	35.0637	34.1519	34.8857	-24.5343	-0.788546	-25.9375	-0	25.9375	-0	1.39052	1.84088	0.521726	2.36719	
42	0.44771	25.7571	38.2878	21.7882	0	8825.18	3.73157	35.1285	33.6986	35.1034	-25.7025	-1.67633	-27.0312	-0	27.0312	-0	1.27416	3.73157	0.491753	2.34838	
43	0.40292	26.986	38.2878	21.7882	0	8826.18	3.75474	35.1725	34.0482	35.1051	-26.928	-1.76719	-28.125	-0	28.125	-0	1.13903	3.75474	0.44944	2.33088	
44	0.482478	28.2711	38.2878	21.7882	0	8827.18	-0.87065	35.217	34.8531	35.2084	-28.2679	0.429583	-29.2188	-0	29.2188	-0	0.947624	0.87065	0.40318	2.43753	
45	0.193719	29.5516	38.2878	21.7881	0	8828.18	2.66937	34.6486	33.8266	34.7313	-29.5195	-1.37629	-30.3125	-0	30.3125	-0	0.760907	2.66937	0.364326	2.43687	
46	-0.200441	30.8813	38.2878	21.7881	0	8829.18	3.49412	33.6414	33.3909	33.4871	-30.8239	-1.88209	-31.4062	-0	31.4062	-0	0.52494	3.49412	0.331196	2.39536	
47	0.721433	32.1289	38.2878	21.7881	0	8830.18	4.21727	34.7397	32.8936	34.5944	-32.042	-2.36272	-32.5	-0	32.5	-0	0.371055	4.21727	0.360084	2.39976	
48	0.325733	33.4563	38.2878	21.7881	0	8831.18	2.95673	34.9405	33.6246	34.6409	-33.4118	-1.72574	-33.5938	-0	33.5938	-0	0.137434	2.95673	0.445097	2.40262	
49	0.483504	34.657	38.2878	21.7881	0	8832.18	-0.160816	35.0583	34.4675	34.5715	-34.6569	0.0972745	-34.6875	-0	34.6875	-0	0.030453	0.160816	0.521046	2.54863	
50	0.0868854	35.8531	38.2878	21.7881	0	8833.18	-1.16668	34.9065	33.2417	34.151	-35.8457	0.730003	-35.7812	-0	35.7812	-0	0.071838	1.16668	0.565093	2.61118	
51	0.229342	37.157	38.2878	21.7881	0	8834.18	5.09111	32.7622	32.0511	33.1832	-37.0104	-3.2973	-36.875	-0	36.875	-0	0.282007	5.09111	0.577788	1.42766	
52	0.445302	38.3742	38.2878	21.788	0	8835.18	0.946485	32.6565	32.0962	32.4981	-38.3689	-0.633884	-37.9688	-0	37.9688	-0	0.405405	0.946485	0.565346	1.51008	
53	0.00988544	39.6312	38.2878	21.788	0	8836.18	2.38511	34.9053	33.1819	34.3384	-39.5968	-1.64929	-39.0625	-0	39.0625	-0	0.56867	2.38511	0.532785	1.51021	
54	0.0730433	40.9562	38.2878	21.788	0	8837.18	1.91287	34.8865	33.2058	34.5538	-40.9334	-1.3671	-40.1562	-0	40.1562	-0	0.799946	1.91287	0.48188	1.52474	
55	0.685243	42.2062	38.2878	21.788	0	8838.18	2.31315	34.78	32.8759	33.4911	-42.1718	-1.70348	-41.25	-0	41.25	-0	0.956176	2.31315	0.436692	1.39193	
56	0.200774	43.4397	38.2878	21.788	0	8839.18	7.49336	32.6793	31.4511	31.2222	-43.0688	-5.66503	-42.3438	-0	42.3438	-0	1.09599	7.49336	0.406293	1.88007	
57	-0.0938923	44.7366	38.2878	21.788	0	8840.18	3.23902	34.7176	33.8313	33.8644	-44.6652	-2.52769	-43.4375	-0	43.4375	-0	1.29912	3.23902	0.409186	1.86835	
58	0.420256	46.0124	38.2878	21.788	0	8841.18	2.97199	31.1087	30.1088	30.5446	-45.9505	-2.38564	-44.5312	-0	44.5312	-0	1.48115	2.97199	0.447558	1.85198	
59	0.456956	47.314	38.2878	21.7879	0	8842.18	0.631113	34.1405	32.6786	33.7282	-47.3111	-0.521153	-45.625	-0	45.625	-0	1.68897	0.631113	0.518257	1.87067	
60	-0.12222	48.5006	38.2878	21.7879	0	8843.18	7.85129	33.7131	32.6741	33.5686	-48.046	-6.6253	-46.7188	-0	46.7188	-0	1.78189	7.85129	0.589253	2.28258	
61	-0.366698	49.767	38.2878	21.7879	0	8844.18	2.34248	34.7232	32.878	33.8068	-49.7254	-2.03411	-47.8125	-0	47.8125	-0	1.95453	2.34248	0.658915	2.28853	
62	-0.657015	51.0311	38.2878	21.7879	0	8845.18	0.930389	34.4722	33.0507	34.2815	-51.0244	-0.828625	-48.9062	-0	48.9062	-0	2.12483	0.930389	0.718544	2.32536	
63	-0.450115	52.3045	38.2878	21.7879	0	8846.18	4.69838	33.0905	32.006	33.3964	-52.1288	-4.28428	-50	0	50	-0	2.30451	4.69838	0.754314	2.3753	
64	0.582473	53.4794	38.2878	21.7879	0	8847.18	1.02401	33.7749	32.5164	33.2699	-53.4709	-0.955748	-51.0938	0	51.0938	-0	2.3857	1.02401	0.75577	2.31273	
65	-0.100922	54.6216	38.2878	21.7879	0	8848.18	0.075714	32.3832	32.3678	32.5673	-54.6215	-0.0721801	-52.1875	0	52.1875	-0	2.43405	0.075714	0.731758	2.39035	
66	0.106435	55.4635	38.2878	21.7879	0	8849.18	9.2498	33.5939	32.7337	31.9775	-54.7423	-8.91515	-53.2812	0	53.2812	-0	2.18222	9.2498	0.680083	2.85524	
67	0.416205	56.5813	38.2878	21.7878	0	8850.18	-7.08382	32.1431	33.0988	32.4013	-56.1494	6.97768	-54.375	0	54.375	-0	2.20634	7.08382	0.616931	2.94684	
68	0.142266	57.9916	38.2878	21.7878	0	8851.18	-8.96393	32.489	33.8099	32.323	-57.2833	9.03582	-55.4688	0	55.4688	-0	2.52282	8.96393	0.568988	3.2272	
69	0.505103	58.8734	38.2878	21.7878	0	8852.18	1.22185	27.9109	29.2966	27.7246	-58.86	-1.25539	-56.5625	0	56.5625	-0	2.31086	1.22185	0.506894	3.26463	
70	0.270755	60.0616	38.2878	21.7878	0	8853.18	15.078	32.1607	31.6561	32.3599	-57.9938	-15.624	-57.6562	0	57.6562	-0	2.40533	15.078	0.445409	4.29343	
71	-0.277658	61.2795	38.2878	21.7878	0	8854.18	2.28247	32.8763	31.9895	31.9735	-61.2309	-2.44052	-58.75	0	58.75	-0	2.52951	2.28247	0.384477	4.27566	
72	0.727078	62.2504	38.2878	21.7878	0	8855.18	-7.97576	32.3937	31.8904	32.2209	-61.6483	8.6375	-59.8438	0	59.8438	-0	2.40667	7.97576	0.318912	4.34939	
73	-0.128448	63.7889	38.2878	21.7878	0	8856.18	10.9768	28.3319	27.6116	28.1228	-62.6218	-12.1461	-60.9375	0	60.9375	-0	2.85135	10.9768	0.2997	4.59016	
74	0.101855	65.3554	38.2878	21.7877	0	8857.18	-1.9767	32.1461	32.1763	33.0308	-65.3165	2.25431	-62.0312	0	62.0312	-0	3.32418	1.9767	0.362954	4.50349	
75	0.280927	66.5257	38.2878	21.7877	0	8858.18	-1.80148	32.7565	32.5566	32.2857	-66.4928	2.09134	-63.125	0	63.125	-0	3.40068	1.80148	0.409555	4.54368	
76	0.28733	67.771	38.2878	21.7877	0	8859.18	2.01122	32.5438	30.8615	33.1104	-67.7292	-2.37844	-64.2188	0	64.2188	-0	3.55222	2.01122	0.464532	4.55854	
77	-0.187231	68.9013	38.2878	21.7877	0	8860.18	8.99386	29.9141	28.2227	30.633	-68.0542	-10.7712	-65.3125	0	65.3125	-0	3.58884	8.99386	0.510018	4.51665	
78	0.175024	69.8019	38.2878	21.7877	0	8861.18	-6.24728	31.8597	33.6009	32.1643	-69.3874	7.59581	-66.4062	0	66.4062	-0	3.39564	6.24728	0.52804	4.51322	
79	0.230587	70.7024	38.2878	21.7877	0	8862.18	0.542648	31.055	29.0121	31.8446	-70.6993	-0.669613	-67.5	0	67.5	-0	3.20244	0.542648	0.528086	4.55013	
80	-0.177059	71.8399	38.2878	21.7877	0	8863.18	3.01107	28.8465	27.9697	31.5818	-71.7407	-3.77367	-68.5938	0	68.5938	-0	3.2461	3.01107	0.527221	4.35295	
81	-0.497823	72.9186	38.2878	21.7876	0	8864.18	-4.25626	31.7792	29.3907	32.443	-72.7175	5.41184	-69.6875	0	69.6875	-0	3.23113	4.25626	0.497493	4.26256	
82	0.16433	73.7277	38.2878	21.7876	0	8865.18	-8.54687	31.3801	30.0451	32.9075	-72.9089	10.9573	-70.7812	0	70.7812	-0	2.94647	8.54687	0.453788	4.31789	
83	-0.115948	74.7877	38.2878	21.7876	0	8866.18	10.4264	31.1922	30.1928	32.034	-73.5529	-13.5345	-71.875	0	71.875	-0	2.91274	10.4264	0.435658	4.41488	
84	0.368139	75.4194	38.2878	21.7876	0	8867.18	9.983	28.2187	25.123	28.8364	-74.2775	-13.0744	-72.9688	0	72.9688	-0	2.45063	9.983	0.420637	4.36075	
85	0.739279	76.0964	38.2878	21.7876	0	8868.18	3.91279	27.6639	24.7823	29.6217	-75.919	-5.19267	-74.0625	0	74.0625	-0	2.03385	3.91279	0.468257	3.64476	
86	0.510052	76.6897	38.2878	21.7876	0	8869.18	4.98629	32.1305	32.2124	32.2134	-76.3994	-6.66567	-75.1562	0	75.1562	-0	1.53343	4.98629	0.594177	3.53799	
87	0.886802	77.4026	38.2878	21.7876	0	8870.18	-1.08408	28.68	23.3602	27.9588	-77.3888	1.46443	-76.25	0	76.25	-0	1.15261	1.08408	0.743743	3.66782	
88	0.571969	78.275	38.2878	21.7876	0	8871.18	5.1876	32.2595	30.8671	32.2944	-77.9544	-7.07739	-77.3438	0	77.3438	-0	0.93127	5.1876	0.894364	3.30929	
89	NaN	79.389	38.2878	21.7876	0	8872.18	11.4536	27.8919	22.1658	27.2065	-77.808	-15.7646	-78.4375	0	78.4375	-0	0.951481	11.4536	0.986265	3.6096	
90	-0.832856	80.4842	38.2878	21.7876	0	8873.18	-0.205168	30.1534	25.2715	27.2735	-80.4837	0.288202	-79.5312	0	79.5312	-0	0.952928	0.205168	1.03981	3.74722	
91	-0.893079	81.645	38.2878	21.7875	0	8874.18	12.9925	28.6597	23.1573	27.8592	-79.5549	-18.3558	-80.625	0	80.625	-0	1.02004	12.9925	1.04587	4.09642	
92	-0.58864	NaN	38.2878	21.7875	0	8875.18	2.07559	32.1444	28.6571	30.3294	NaN	NaN	-81.7188	0	81.7188	-0	NaN	2.07559	1.01355	4.13922	
93	-0.849812	83.7369	38.2878	21.7875	0	8876.18	5.38946	32.2874	29.3976	31.6849	-83.3668	-7.86501	-82.8125	0	82.8125	-0	0.924441	5.38946	0.993039	4.13646	
94	-1.35491	84.4921	38.2878	21.7875	0	8877.18	9.34762	32.5806	30.0314	31.8314	-83.3701	-13.7235	-83.9062	0	83.9062	-0	0.585838	9.34762	0.988153	3.9891	
95	-0.750253	85.2637	38.2878	21.7875	0	8878.18	7.32847	32.7019	30.5548	32.7713	-84.5671	-10.876	-85	0	85	-0	0.263653	7.32847	0.968276	3.89802	
96	-0.53967	85.8523	38.2878	21.7875	0	8879.18	5.64046	32.4857	28.546	32.527	-85.4366	-8.43805	-85	0	85	-0	0.852292	5.64046	0.855272	3.85784	
97	-1.22123	86.3964	38.2878	21.7875	0	8880.18	9.51588	32.6081	30.0177	32.961	-85.2075	-14.2831	-85	0	85	-0	1.39637	9.51588	0.729944	3.90116	
98	-1.72049	NaN	38.2878	21.7875	0	8881.18	10.2795	32.6999	29.4862	32.1459	NaN	NaN	-85	0	85	-0	NaN	10.2795	0.582106	3.89114	
99	-0.39384	NaN	38.2878	21.7875	0	8882.18	8.54338	24.9493	23.4866	24.3811	NaN	NaN	-85	0	85	-0	NaN	8.54338	0.452763	3.81951	
100	-1.15606	NaN	38.2878	21.7875	0	8883.18	7.42134	27.7539	26.0049	27.0318	NaN	NaN	-85	0	85	-0	NaN	7.42134	0.346216	3.7547	
101	-1.27078	NaN	38.2878	21.7875	0	8884.18	6.31129	32.9318	29.5459	32.1919	NaN	NaN	-85	0	85	-0	NaN	6.31129	0.305042	3.72538	
102	-0.964948	NaN	38.2878	21.7875	0	8885.18	6.58025	32.569	29.4273	32.0267	NaN	NaN	-85	0	85	-0	NaN	6.58025	0.309894	3.37101	
103	-1.99436	NaN	38.2878	21.7875	0	8886.18	5.04547	31.999	27.8633	31.7905	NaN	NaN	-85	0	85	-0	NaN	5.04547	0.330532	3.37732	
104	-0.599062	86.3026	38.2878	21.7875	0	8887.18	3.19251	31.914	28.0457	31.7962	-86.1686	-4.80628	-85	0	85	-0	1.30257	3.19251	0.364685	3.30852	
105	-1.3138	86.3753	38.2878	21.7875	0	8888.18	6.55753	32.236	28.6378	32.1129	-85.8102	-9.86413	-85	0	85	-0	1.37527	6.55753	0.400247	2.7894	
106	-0.857892	86.3776	38.2878	21.7875	0	8889.18	4.96317	27.5588	24.6395	26.7516	-86.0537	-7.47299	-85	0	85	-0	1.37761	4.96317	0.426376	2.30183	
107	-1.09116	86.3471	38.2878	21.7875	0	8890.18	4.86293	32.4313	28.6174	32.0528	-86.0363	-7.31985	-85	0	85	-0	1.34713	4.86293	0.41439	2.00904	
108	-1.27495	86.3307	38.2878	21.7875	0	8891.18	7.03188	32.7444	29.2216	32.5235	-85.6813	-10.5687	-85	0	85	-0	1.33071	7.03188	0.421409	1.97512	
109	-0.677281	86.3401	38.2878	21.7875	0	8892.18	5.48749	23.4993	21.7032	22.7494	-85.9444	-8.25656	-85	0	85	-0	1.34009	5.48749	0.381157	1.87415	
110	-1.17311	86.319	38.2878	21.7875	0	8893.18	7.04757	32.9168	29.4899	32.7021	-85.6668	-10.5908	-85	0	85	-0	1.31898	7.04757	0.168141	1.86757	
111	-0.622198	86.3401	38.2878	21.7875	0	8894.18	3.64798	32.4618	28.3421	31.7574	-86.1651	-5.4935	-85	0	85	-0	1.34009	3.64798	0.0301878	2.00394	
112	-0.584458	NaN	38.2878	21.7875	0	8895.18	7.14502	32.5864	28.7701	32.0334	NaN	NaN	-85	0	85	-0	NaN	7.14502	0.0256882	1.82926	
113	-1.16686	86.054	38.2878	21.7875	0	8896.18	8.88104	26.8164	24.5598	25.8609	-85.0223	-13.2853	-85	0	85	-0	1.05398	8.88104	0.0988251	1.63598	
114	-0.844033	85.2379	38.2878	21.7875	0	8897.18	-2.62575	31.8233	29.0225	31.8198	-85.1484	3.90491	-85	0	85	-0	0.237855	2.62575	0.35149	1.73612	
115	-0.542084	NaN	38.2878	21.7875	0	8898.18	9.65678	31.3318	28.3904	31.2233	NaN	NaN	-85	0	85	-0	NaN	9.65678	0.35149	1.96704	
116	-0.59538	NaN	38.2878	21.7875	0	8899.18	-3.81578	32.2118	28.5072	31.3009	NaN	NaN	-85	0	85	-0	NaN	3.81578	0.35149	2.03729	
117	-1.17645	NaN	38.2878	21.7875	0	8900.18	-0.541546	31.4688	28.2366	31.605	NaN	NaN	-83.75	-0	83.75	-0	NaN	0.541546	0.35149	2.42531	
118	-1.07897	80.51	38.2878	21.7875	0	8901.18	4.81362	31.6225	28.4107	31.819	-80.226	-6.75597	-82.5	0	82.5	-0	1.99002	4.81362	0.409368	2.42824	
119	-1.24865	80.388	38.2878	21.7875	0	8902.18	5.61148	23.3278	22.0391	23.4006	-80.0028	-7.86053	-81.25	0	81.25	-0	0.861974	5.61148	0.427452	2.35381	
120	-0.51222	80.388	38.2878	21.7875	0	8903.18	5.52243	31.4788	27.9865	31.6683	-80.0149	-7.73618	-80	0	80	-0	0.388026	5.52243	0.493377	2.33609	
121	-0.893303	80.4584	38.2878	21.7875	0	8904.18	2.88216	32.1331	28.7213	31.9663	-80.3566	-4.0456	-80	0	80	-0	0.458382	2.88216	0.526621	2.4267	
122	-1.35278	80.4021	38.2878	21.7875	0	8905.18	5.62701	31.2797	27.7971	31.123	-80.0147	-7.8836	-80	0	80	-0	0.402097	5.62701	0.551702	2.42478	
123	-1.49595	80.449	38.2878	21.7875	0	8906.18	5.91242	30.6846	27.2312	30.6691	-80.0211	-8.28691	-80	0	80	-0	0.449001	5.91242	0.558818	2.38643	
124	-0.364073	NaN	38.2878	21.7875	0	8907.18	4.04579	31.5705	28.3543	31.2222	NaN	NaN	-80	0	80	-0	NaN	4.04579	0.568082	2.40648	
125	-0.731365	NaN	38.2878	21.7876	0	8908.18	5.52945	31.5812	27.9525	31.2924	NaN	NaN	-80	0	80	-0	NaN	5.52945	0.576641	2.3539	
126	-0.308865	80.5428	38.2878	21.7876	0	8909.18	5.40132	31.6868	28.0582	31.5168	-80.1852	-7.58159	-80	0	80	-0	0.542808	5.40132	0.543214	2.32081	
127	-0.576837	80.4584	38.2878	21.7876	0	8910.18	6.04251	31.8088	28.7132	31.6174	-80.0114	-8.46955	-80	0	80	-0	0.458382	6.04251	0.51826	2.27178	
128	-0.759998	NaN	38.2878	21.7876	0	8911.18	8.98306	30.8052	26.6927	29.4313	NaN	NaN	-80	0	80	-0	NaN	8.98306	0.532148	2.28394	
129	-0.954559	80.4584	38.2878	21.7876	0	8912.18	-4.5315	29.5059	27.0197	30.5996	-80.2069	6.35678	-80	0	80	-0	0.458382	4.5315	0.515984	2.18532	
130	-1.0298	80.2567	38.2878	21.7876	0	8913.18	-1.83808	30.1773	28.7505	30.9469	-80.2154	2.57423	-80	0	80	-0	0.256696	1.83808	0.503535	1.98528	
131	-0.723607	80.2004	38.2878	21.7876	0	8914.18	8.02238	32.4266	27.5074	29.8375	-79.4155	-11.1928	-80	0	80	-0	0.200412	8.02238	0.494675	2.13675	
132	-1.07118	80.3224	38.2878	21.7876	0	8915.18	5.60668	32.599	28.925	30.5552	-79.9381	-7.84741	-80	0	80	-0	0.322361	5.60668	0.47784	1.7422	
133	-0.793079	80.3622	38.2878	21.7876	0	8916.18	5.11332	32.8223	30.0685	32.8939	-80.0424	-7.16236	-80	0	80	-0	0.362229	5.11332	0.166124	1.73722	
134	-1.05945	80.5545	38.2878	21.7876	0	8917.18	5.84614	32.3297	31.9788	32.1945	-80.1356	-8.20508	-80	0	80	-0	0.554534	5.84614	0.106446	1.74053	
135	-1.38623	80.6554	38.2878	21.7876	0	8918.18	4.20777	31.7123	27.6965	30.6978	-80.438	-5.91797	-80	0	80	-0	0.655377	4.20777	0.12841	1.76649	
136	-0.554357	80.7656	38.2878	21.7876	0	8919.18	12.7102	32.3497	27.7871	32.1201	-78.7865	-17.77	-80	0	80	-0	0.7656	12.7102	0.161626	2.48128	
137	-1.457	80.9321	38.2877	21.7876	0	8920.18	3.32257	28.6322	24.5301	26.7281	-80.7961	-4.69061	-80	-1.84211	80.0212	1.31908	0.910902	2.00349	0.207485	2.68422	
138	-0.654305	81.2464	38.2877	21.7876	0	8921.18	5.3243	25.5921	25.7713	27.5076	-80.8958	-7.53909	-80	-3.68421	80.0848	2.63676	1.16157	2.68755	0.28185	2.79455	
139	-1.15048	81.4058	38.2877	21.7876	0	8922.18	8.39655	29.7882	28.149	30.1216	-80.5333	-11.8872	-80	-5.52632	80.1906	3.95165	1.21519	4.4449	0.326247	2.78154	
140	-0.666685	81.638	38.2877	21.7876	0	8923.18	9.38925	32.7319	31.6812	32.6546	-80.5443	-13.3185	-80	-7.36842	80.3386	5.2624	1.29939	4.12685	0.364273	2.80508	
141	-0.748248	81.8233	38.2877	21.7876	0	8924.18	8.94223	32.7094	30.4919	33.1928	-80.8288	-12.7185	-80	-9.21053	80.5285	6.56764	1.29481	2.3746	0.400199	2.91461	
142	-1.15913	NaN	38.2877	21.7876	0	8925.18	10.2948	32.089	31.2194	32.8311	NaN	NaN	-80	-11.0526	80.7599	7.86607	NaN	2.42875	0.409758	2.99152	
143	-0.820524	82.3298	38.2877	21.7876	0	8926.18	10.3273	24.1938	22.9847	28.0146	-80.9961	-14.7594	-80	-12.8947	81.0326	9.15642	1.29728	1.17092	0.422109	2.92696	
144	-0.505337	NaN	38.2877	21.7876	0	8927.18	12.3727	26.5953	24.193	27.8011	NaN	NaN	-80	-14.7368	81.346	10.4375	NaN	1.93526	0.42943	2.9992	
145	-0.430266	NaN	38.2877	21.7876	0	8928.18	13.698	22.043	19.487	23.9823	NaN	NaN	-80	-16.5789	81.6998	11.7081	NaN	1.98991	0.415874	2.99054	
146	-1.27789	NaN	38.2877	21.7876	0	8929.18	14.3127	25.843	21.6892	23.8443	NaN	NaN	-80	-18.4211	82.0935	12.9671	NaN	1.34562	0.382214	2.89404	
147	-0.961742	NaN	38.2877	21.7875	0	8930.18	17.7902	29.5595	27.7813	30.2353	NaN	NaN	-80	-20.2632	82.5263	14.2135	NaN	3.57675	0.349735	2.85402	
148	-0.687117	NaN	38.2876	21.7875	0	8931.18	15.1813	29.8338	26.8481	31.7142	NaN	NaN	-80	-22.1053	82.9978	15.4463	NaN	0.265046	0.298907	2.95888	
149	-1.22713	NaN	38.2876	21.7875	0	8932.18	16.6712	32.9425	29.3646	32.8882	NaN	NaN	-80	-23.9474	83.5073	16.6647	NaN	0.00651925	0.26021	2.99901	
150	-0.7294	NaN	38.2876	21.7875	0	8933.18	18.202	32.466	32.4567	33.148	NaN	NaN	-80	-25.7895	84.0541	17.8677	NaN	0.334272	0.213194	3.0555	
151	-0.762251	NaN	38.2876	21.7875	0	8934.18	15.248	31.2193	27.0362	31.0714	NaN	NaN	-80	-27.6316	84.6375	19.0546	NaN	3.80662	0.150694	1.40181	
152	-0.830519	NaN	38.2876	21.7875	0	8935.18	15.0123	32.0639	27.1001	31.7874	NaN	NaN	-80	-29.4737	85.2567	20.2249	NaN	5.2126	0.0625453	1.60527	
153	-1.3335	84.4968	38.2876	21.7875	0	8936.18	18.4633	32.5347	28.5175	32.361	-80.1474	-26.7599	-80	-31.3158	85.9109	21.3777	1.4141	2.91442	0.0709933	1.60944	
154	-1.39956	85.9649	38.2876	21.7875	0	8937.18	16.3583	32.5979	28.9968	33.0482	-82.4849	-24.2114	-80	-33.1579	86.5993	22.5127	0.634481	6.15444	0.313553	1.81263	
155	-0.981448	NaN	38.2876	21.7875	0	8938.18	16.9442	32.7279	32.1221	32.5779	NaN	NaN	-80	-35	87.3212	23.6294	NaN	6.68517	0.35485	2.07679	
156	-0.427009	NaN	38.2876	21.7875	0	8939.18	20.7995	30.6398	28.3847	31.0378	NaN	NaN	-80	-35	87.3212	23.6294	NaN	2.82985	0.420467	2.07533	
157	-0.747329	NaN	38.2875	21.7875	0	8940.18	20.4875	32.2794	26.8228	32.638	NaN	NaN	-80	-35	87.3212	23.6294	NaN	3.14183	0.420467	2.07658	
158	-0.177366	87.3602	38.2875	21.7875	0	8941.18	22.4506	33.1227	30.5286	33.1901	-80.7391	-33.3617	-80	-35	87.3212	23.6294	0.0389955	1.17877	0.689603	2.07616	
159	-0.653341	NaN	38.2875	21.7875	0	8942.18	19.7466	21.3995	22.2861	20.8743	NaN	NaN	-80	-35	87.3212	23.6294	NaN	3.88277	0.689603	2.08189	
160	-1.01589	NaN	38.2875	21.7875	0	8943.18	22.2636	26.912	26.0821	26.179	NaN	NaN	-80	-35	87.3212	23.6294	NaN	1.36577	0.689603	2.10721	
161	-0.952892	87.4001	38.2875	21.7876	0	8944.18	18.4921	23.5223	22.358	23.5304	-82.8874	-27.721	-80	-35	87.3212	23.6294	0.078864	5.13728	0.642032	2.14142	
162	-0.967115	87.3485	38.2875	21.7876	0	8945.18	17.586	31.7484	30.2275	33.4935	-83.2662	-26.3912	-80	-35	87.3212	23.6294	0.02727	6.04338	0.601716	2.27145	
163	-1.39734	87.4939	38.2875	21.7876	0	8946.18	18.3714	32.8291	31.8211	32.4488	-83.0347	-27.5759	-80	-35	87.3212	23.6294	0.172671	5.25801	0.549044	2.16389	
164	-0.837892	87.3907	38.2875	21.7876	0	8947.18	14.3727	29.1974	26.9848	30.7533	-84.6555	-21.6929	-80	-35	87.3212	23.6294	0.069483	9.25667	0.516032	2.37538	
165	-0.811343	87.4376	38.2875	21.7876	0	8948.18	12.9319	28.0035	26.1495	30.2305	-85.2199	-19.5678	-80	-35	87.3212	23.6294	0.116387	10.6975	0.484718	2.65692	
166	-0.756642	87.3931	38.2875	21.7875	0	8949.18	13.8913	28.521	26.5179	30.474	-84.8371	-20.9813	-80	-35	87.3212	23.6294	0.0718285	9.7381	0.460839	2.91111	
167	-0.383448	87.4353	38.2876	21.7875	0	8950.18	13.0606	28.2165	26.2369	30.3871	-85.1735	-19.7587	-80	-35	87.3212	23.6294	0.114042	10.5688	0.438095	3.21255	
168	-0.730115	87.372	38.2876	21.7876	0	8951.18	13.7159	26.1608	24.5895	27.2546	-84.8804	-20.7166	-80	-35	87.3212	23.6294	0.0507215	9.91348	0.17981	3.29305	
169	-0.701683	87.4658	38.2876	21.7876	0	8952.18	14.5341	23.6973	22.4452	24.4009	-84.6667	-21.9501	-80	-35	87.3212	23.6294	0.144529	9.09524	0.0471564	3.38139	
170	-1.27886	87.5103	38.2876	21.7876	0	8953.18	15.0442	28.4373	25.8234	28.7231	-84.511	-22.7145	-80	-35	87.3212	23.6294	0.189087	8.58522	0.0540512	3.43128	
171	-0.897998	87.454	38.2875	21.7876	0	8954.18	14.0499	29.6913	26.7769	30.3205	-84.8378	-21.2309	-80	-35	87.3212	23.6294	0.132803	9.57949	0.0525267	3.3651	
172	-0.771971	87.4892	38.2875	21.7876	0	8955.18	12.7603	29.0774	26.5154	30.0629	-85.3285	-19.324	-80	-35	87.3212	23.6294	0.167981	10.8691	0.0536547	3.34069	
173	-0.810281	87.4212	38.2875	21.7875	0	8956.18	14.6753	29.6017	27.0359	31.351	-84.5693	-22.1474	-80	-35	87.3212	23.6294	0.0999705	8.95405	0.0498649	2.87536	
174	-0.835813	87.5549	38.2875	21.7875	0	8957.18	14.6812	28.4127	26.6553	30.6128	-84.6963	-22.19	-80	-35	87.3212	23.6294	0.233646	8.94814	0.0581344	2.65515	
175	-0.974559	87.3368	38.2875	21.7875	0	8958.18	22.0009	31.847	30.8489	32.9527	-80.9767	-32.7182	-80	-35	87.3212	23.6294	0.015544	1.62847	0.0620886	2.6068	
176	-1.07572	86.7364	38.2875	21.7875	0	8959.18	21.9111	32.5165	29.8722	32.348	-80.4709	-32.3672	-80	-35	87.3212	23.6294	0.584822	1.71826	0.136025	3.01863	
177	-0.710245	85.7374	38.2875	21.7876	0	8960.18	14.8117	32.6602	30.5429	32.8582	-82.8884	-21.9182	-78.5227	-35	85.9699	24.024	0.232493	9.21229	0.133522	2.97826	
178	-0.74967	84.1028	38.2875	21.7876	0	8961.18	19.1853	32.0926	27.3512	30.6213	-79.4318	-27.6382	-77.0455	-35	84.6227	24.4312	0.519915	5.24593	0.162815	2.97913	
179	0.0792091	83.3265	38.2875	21.7876	0	8962.18	23.4072	25.4909	22.3863	25.0753	-76.4691	-33.1026	-75.5682	-35	83.28	24.8516	0.0465848	1.44435	0.164056	3.44093	
180	-0.444698	NaN	38.2875	21.7876	0	8963.18	16.1647	23.1335	21.3416	22.6516	NaN	NaN	-74.0909	-35	81.9418	25.2857	NaN	9.12096	0.169225	3.36765	
181	-0.984956	NaN	38.2875	21.7877	0	8964.18	8.4228	24.3198	21.2171	24.5759	NaN	NaN	-72.6136	-35	80.6086	25.7342	NaN	17.3114	0.172782	4.17529	
182	-0.266726	NaN	38.2875	21.7877	0	8965.18	23.883	27.6804	26.5138	29.982	NaN	NaN	-71.1364	-35	79.2804	26.1978	NaN	2.31476	0.178677	4.37248	
183	-0.520699	NaN	38.2875	21.7877	0	8966.18	25.7323	31.696	28.7513	30.816	NaN	NaN	-69.6591	-35	77.9576	26.6771	NaN	0.944833	0.180659	4.63809	
184	-1.24946	NaN	38.2875	21.7877	0	8967.18	24.6973	29.4425	27.4263	32.2168	NaN	NaN	-68.1818	-35	76.6405	27.1729	NaN	2.47569	0.188821	4.73815	
185	-0.399559	NaN	38.2875	21.7878	0	8968.18	29.198	28.8458	25.6593	28.5536	NaN	NaN	-66.7045	-35	75.3293	27.6861	NaN	1.51191	0.199893	4.87195	
186	-0.802448	NaN	38.2875	21.7878	0	8969.18	26.4947	31.4386	30.9089	32.3266	NaN	NaN	-65.2273	-35	74.0243	28.2174	NaN	1.72269	0.210405	4.89176	
187	-0.785801	73.8309	38.2875	21.7878	0	8970.18	29.0199	32.9376	33.7834	32.3718	-64.5615	-35.8163	-63.75	-35	72.7259	28.7676	1.10497	0.252238	0.367927	4.83672	
188	-0.878948	72.588	38.2875	21.7878	0	8971.18	26.3537	33.2912	33.0574	32.8107	-65.0439	-32.2226	-62.2727	-35	71.4345	29.3379	1.15343	2.98419	0.444307	4.71942	
189	-0.335073	71.3802	38.2875	21.7878	0	8972.18	25.0984	32.8679	33.0765	32.8761	-64.6405	-30.2776	-60.7955	-35	70.1505	29.9291	1.22973	4.83067	0.499492	4.55639	
190	-0.865499	70.1654	38.2875	21.7878	0	8973.18	26.7564	33.2133	33.124	32.7692	-62.6527	-31.5883	-59.3182	-35	68.8741	30.5422	1.29126	3.78584	0.485704	4.5038	
191	-0.632539	68.9998	38.2875	21.7878	0	8974.18	28.385	30.9577	29.9656	31.8874	-60.7042	-32.8021	-57.8409	-35	67.606	31.1785	1.39384	2.79344	0.524239	4.46776	
192	-0.617418	67.717	38.2875	21.7878	0	8975.18	24.2712	32.1416	27.9445	30.4142	-61.7315	-27.8355	-56.3636	-35	66.3465	31.8389	1.37052	7.56778	0.478468	4.36003	
193	0.24438	66.5773	38.2875	21.7878	0	8976.18	25.0083	32.5047	32.3378	32.5326	-60.3354	-28.1455	-54.8864	-35	65.0962	32.5249	1.48109	7.51664	0.456933	4.43448	
194	-0.144698	65.3976	38.2875	21.7878	0	8977.18	34.7193	29.6341	28.5573	30.699	-53.7538	-37.2476	-53.4091	-35	63.8555	33.2376	1.5421	1.48168	0.154103	4.43269	
195	-0.828281	NaN	38.2875	21.7879	0	8978.18	33.867	31.5394	28.0553	32.1871	NaN	NaN	-51.9318	-35	62.6252	33.9784	NaN	0.111462	0.154103	4.3631	
196	-0.505769	63.817	38.2875	21.7879	0	8979.18	38.6223	31.4361	30.2985	31.7941	-49.8588	-39.8335	-50.4545	-35	61.4057	34.7488	2.41129	3.87351	0.391014	2.28358	
197	-0.568607	62.0487	38.2875	21.7879	0	8980.18	33.455	32.5666	29.6979	33.2341	-51.7684	-34.2064	-48.9773	-35	60.1978	35.5503	1.85095	2.09522	0.390674	2.28861	
198	-0.960198	60.6721	38.2875	21.7879	0	8981.18	32.7214	33.5485	32.757	33.724	-51.044	-32.7966	-47.5	-35	59.0021	36.3844	1.66999	3.66299	0.374893	2.22699	
199	-0.655353	59.5066	38.2875	21.7879	0	8982.18	34.3128	32.807	32.8847	32.9072	-49.1508	-33.5445	-46.0227	-35	57.8195	37.2528	1.68708	2.93999	0.361507	2.22074	
200	-0.404016	58.2988	38.2875	21.7879	0	8983.18	27.7785	32.0058	30.972	32.2498	-51.5802	-27.1705	-44.5455	-35	56.6507	38.1572	1.64813	10.3787	0.348065	2.84749	
201	-0.0540035	57.1497	38.2875	21.7879	0	8984.18	32.7812	33.7362	31.9946	33.6242	-48.0482	-30.9427	-43.0682	-35	55.4966	39.0995	1.65309	6.3183	0.336138	2.86292	
202	-0.73567	56.0967	38.2875	21.7879	0	8985.18	37.0786	33.2356	32.9434	33.5352	-44.7545	-33.8212	-41.5909	-35	54.3581	40.0816	1.73856	3.00306	0.315853	2.6856	
203	-0.703382	54.9217	38.2875	21.7879	0	8986.18	44.4236	32.955	33.1064	33.2772	-39.2243	-38.4429	-40.1136	-35	53.2363	41.1054	1.68543	3.3182	0.29165	2.67596	
204	-0.508231	53.7749	38.2875	21.788	0	8987.18	46.0784	33.5185	33.0876	34.6211	-37.3023	-38.7335	-38.6364	-35	52.1322	42.1729	1.64272	3.90551	0.269386	2.67216	
205	-0.250531	52.729	38.2875	21.788	0	8988.18	37.6229	34.4324	32.7341	34.319	-41.7638	-32.189	-37.1591	-35	51.047	43.2861	1.68197	5.66326	0.249107	2.69607	
206	NaN	51.6338	38.2875	21.788	0	8989.18	37.5906	32.6421	31.8904	32.9465	-40.9141	-31.4974	-35.6818	-35	49.9819	44.4473	1.65188	6.85673	0.23586	2.73678	
207	2.0248	50.5878	38.2875	21.788	0	8990.18	28.0133	32.7193	31.529	32.702	-44.6609	-23.7599	-34.2045	-35	48.9382	45.6585	1.64961	17.6452	0.217504	4.30839	
208	1.2579	49.5958	38.2875	21.788	0	8991.18	36.8806	31.0704	28.7995	31.1416	-39.6711	-29.7649	-32.7273	-35	47.9174	46.922	1.67846	10.0413	0.207419	4.45019	
209	0.97712	48.5898	38.2875	21.788	0	8992.18	44.9036	31.7607	30.9054	32.1321	-34.4159	-34.3003	-31.25	-35	46.9208	48.2397	1.66894	3.33612	0.201358	4.35778	
210	1.26445	47.851	38.2875	21.788	0	8993.18	36.548	31.7876	32.9687	32.4357	-38.4415	-28.4951	-29.7727	-35	45.9501	49.6139	1.90088	13.0659	0.198594	4.48617	
211	1.23717	46.3079	38.2875	21.788	0	8994.18	39.8049	32.4855	33.4272	33.3963	-35.575	-29.6452	-28.2955	-35	45.007	51.0465	1.30086	11.2416	0.128113	4.59111	
212	0.808052	45.6161	38.2875	21.788	0	8995.18	42.9237	33.3756	33.2292	33.5082	-33.4029	-31.0656	-26.8182	-35	44.0933	52.5394	1.52281	9.61574	0.123661	4.4372	
213	1.41822	44.6123	38.2875	21.7881	0	8996.18	45.7927	33.5661	33.2175	33.9063	-31.1063	-31.9791	-25.3409	-35	43.2107	54.0945	1.40166	8.30182	0.139296	4.31824	
214	0.52433	NaN	38.2875	21.7881	0	8997.18	45.5065	32.2588	30.5987	32.3757	NaN	NaN	-23.8636	-35	42.3612	55.7131	NaN	10.2066	0.143753	4.14934	
215	0.918997	NaN	38.2875	21.7881	0	8998.18	54.5887	31.1275	27.5145	31.5971	NaN	NaN	-22.3864	-35	41.547	57.3966	NaN	2.80793	0.149528	4.3214	
216	1.14771	NaN	38.2875	21.7881	0	8999.18	57.2997	31.2915	25.1926	31.6546	NaN	NaN	-20.9091	-35	40.77	59.1458	NaN	1.8461	0.155994	4.56982	
217	0.941885	NaN	38.2875	21.7881	0	9000.18	63.6714	31.8845	30.6718	33.765	NaN	NaN	-19.4318	-35	40.0324	60.9612	NaN	2.71024	0.159403	4.59048	
218	1.111	39.4975	38.2875	21.7881	0	9001.18	56.356	31.8101	28.5973	33.7996	-21.8828	-32.8815	-17.9545	-35	39.3366	62.8428	0.160925	6.48675	0.46452	4.46177	
219	0.587825	39.0824	38.2875	21.7881	0	9002.18	55.26	26.9737	22.9713	28.8867	-22.2713	-32.1158	-16.4773	-35	38.6846	64.7899	0.39777	9.52995	0.561896	4.36603	
220	0.658197	NaN	38.2875	21.7881	0	9003.18	51.0132	26.3744	25.1905	26.7555	NaN	NaN	-15	-35	38.0789	66.8014	NaN	15.7882	0.581836	4.75172	
221	1.11468	38.3507	38.2875	21.7882	0	9004.18	59.2998	30.0775	29.8956	31.6728	-19.5798	-32.9759	-15	-35	38.0789	66.8014	0.271837	7.50165	0.656742	4.7374	
222	0.676969	NaN	38.2875	21.7882	0	9005.18	65.0376	30.5095	27.3305	30.7829	NaN	NaN	-15	-35	38.0789	66.8014	NaN	1.76376	0.675697	4.34813	
223	0.741552	37.7175	38.2875	21.7882	0	9006.18	68.9378	27.9197	26.1193	29.5071	-13.555	-35.1976	-15	-35	38.0789	66.8014	0.361361	2.13637	0.688208	4.50928	
224	0.945774	37.1711	38.2875	21.7882	0	9007.18	67.2557	25.891	26.2821	29.3102	-14.371	-34.2806	-15	-35	38.0789	66.8014	0.907788	0.454324	0.640654	4.73628	
225	0.517348	NaN	38.2875	21.7882	0	9008.18	56.7652	32.7194	32.3724	32.1461	NaN	NaN	-15	-35	38.0789	66.8014	NaN	10.0362	0.559056	4.51379	
226	1.125	NaN	38.2875	21.7882	0	9009.18	61.4118	32.1326	32.3781	32.7582	NaN	NaN	-15	-35	38.0789	66.8014	NaN	5.3896	0.561289	4.34241	
227	0.0565521	NaN	38.2875	21.7882	0	9010.18	54.0045	28.2802	27.2219	27.7337	NaN	NaN	-15	-35	38.0789	66.8014	NaN	12.7969	0.476256	4.58647	
228	0.899302	NaN	38.2875	21.7882	0	9011.18	61.4351	32.4777	32.1085	32.5387	NaN	NaN	-15	-35	38.0789	66.8014	NaN	5.36629	0.287637	4.56747	
229	0.940597	37.1429	38.2875	21.7882	0	9012.18	58.9287	31.2735	30.4894	31.5186	-19.1697	-31.8139	-15	-35	38.0789	66.8014	0.93593	7.87275	0.33251	4.46425	
230	0.897802	37.0867	38.2875	21.7882	0	9013.18	65.8738	25.6732	24.7043	26.3983	-15.1591	-33.847	-15	-35	38.0789	66.8014	0.992214	0.927613	0.354848	4.58991	
231	0.636671	37.028	38.2875	21.7882	0	9014.18	66.5199	30.6066	29.1982	31.3194	-14.7531	-33.962	-15	-35	38.0789	66.8014	1.05084	0.281557	0.369031	4.70828	
232	0.000658383	37.0562	38.2875	21.7882	0	9015.18	66.737	30.9002	29.306	31.5707	-14.6354	-34.0436	-15	-35	38.0789	66.8014	1.0227	0.0644373	0.368615	4.88404	
233	1.0885	37.082	38.2875	21.7882	0	9016.18	68.1713	31.8912	30.1658	32.9794	-13.7883	-34.4232	-15	-35	38.0789	66.8014	0.996904	1.3699	0.324772	5.00679	
234	0.446433	37.0491	38.2875	21.7882	0	9017.18	67.7572	31.7875	30.0679	32.6842	-14.0243	-34.2922	-15	-35	38.0789	66.8014	1.02974	0.955813	0.30152	4.99331	
235	1.04983	NaN	38.2875	21.7882	0	9018.18	63.7752	28.4581	27.5694	29.1055	NaN	NaN	-15	-35	38.0789	66.8014	NaN	3.02617	0.30152	3.98041	
236	0.738497	37.1148	38.2875	21.7882	0	9019.18	63.3125	30.6364	29.1708	31.4	-16.6692	-33.1609	-15	-35	38.0789	66.8014	0.964072	3.48892	0.213665	3.86105	
237	0.815037	37.0702	38.2875	21.7882	0	9020.18	69.6918	31.1536	29.7086	31.6349	-12.866	-34.7659	-15	-35	38.0789	66.8014	1.00863	2.89036	0.203476	3.83093	
238	1.06486	37.0515	38.2875	21.7882	0	9021.18	74.5845	32.4698	30.7747	32.945	-9.84891	-35.7185	-15	-35	38.0789	66.8014	1.02739	7.78309	0.0451808	3.9315	
239	0.838983	37.0351	38.2875	21.7882	0	9022.18	70.6047	32.05	30.5715	32.9048	-12.2987	-34.9333	-15	-35	38.0789	66.8014	1.04381	3.8033	0.0360138	3.7976	
240	1.13905	37.0093	38.2875	21.7882	0	9023.18	64.8287	27.9803	26.5457	28.3206	-15.741	-33.4949	-15	-35	38.0789	66.8014	1.0696	1.97267	0.0390008	3.50258	
241	0.880885	NaN	38.2875	21.7882	0	9024.18	63.1093	25.8998	26.0124	26.7981	NaN	NaN	-15	-35	38.0789	66.8014	NaN	3.69211	0.0390008	3.47716	
242	0.555927	36.9928	38.2875	21.7882	0	9025.18	70.6923	31.522	30.7239	32.914	-12.2314	-34.9122	-15	-35	38.0789	66.8014	1.08602	3.89086	0.0427599	2.42317	
243	0.695239	37.0679	38.2875	21.7882	0	9026.18	65.9712	32.2748	31.2338	33.0824	-15.0939	-33.8556	-15	-35	38.0789	66.8014	1.01098	0.830252	0.0409998	2.41105	
244	1.08631	37.1148	38.2875	21.7882	0	9027.18	66.5223	31.4112	29.8864	31.9681	-14.7862	-34.0423	-15	-35	38.0789	66.8014	0.964072	0.27911	0.0368133	2.05327	
245	-0.104698	37.0069	38.2875	21.7882	0	9028.18	76.8524	28.8519	26.4649	30.9955	-8.41758	-36.0369	-15	-35	38.0789	66.8014	1.07195	10.051	0.0383131	2.81259	
246	0.518482	36.9272	38.2875	21.7882	0	9029.18	70.265	28.6855	22.3333	28.629	-12.4692	-34.7582	-15	-35	38.0789	66.8014	1.15169	3.46363	0.0515406	2.71454	
247	0.398289	NaN	38.2875	21.7882	0	9030.18	65.6848	33.0615	32.3825	34.234	NaN	NaN	-15	-33.7037	36.8909	66.0083	NaN	0.323459	0.0537065	2.69412	
248	0.453219	35.1167	38.2875	21.7882	0	9031.18	63.6517	32.0506	30.4633	32.8719	-15.5857	-31.4685	-15	-32.4074	35.7105	65.1626	0.593801	1.51092	0.138734	2.68756	
249	0.264346	34.3944	38.2875	21.7882	0	9032.18	65.1725	31.8363	29.0415	31.4086	-14.4418	-31.2155	-15	-31.1111	34.5384	64.2593	0.144015	0.913251	0.283064	2.69011	
250	0.700408	33.2241	38.2875	21.7882	0	9033.18	69.7248	32.261	29.2819	32.1697	-11.5132	-31.1655	-15	-29.8148	33.3755	63.2928	0.151345	6.43198	0.346191	2.81568	
251	1.18089	32.0914	38.2875	21.7882	0	9034.18	54.824	32.0858	32.7437	34.0955	-18.4876	-26.2311	-15	-28.5185	32.2228	62.2568	0.131333	7.43282	0.399866	3.00048	
252	1.01199	30.9775	38.2875	21.7882	0	9035.18	67.0869	33.4249	32.9117	33.5261	-12.0606	-28.5332	-15	-27.2222	31.0813	61.1443	0.103873	5.94259	0.438217	3.04593	
253	0.815779	30.1731	38.2875	21.7882	0	9036.18	52.0684	31.9819	32.7191	32.4679	-18.548	-23.7989	-15	-25.9259	29.9525	59.9476	0.220543	7.87917	0.450266	3.05479	
254	0.726435	28.7472	38.2875	21.7882	0	9037.18	45.9316	33.8085	32.7051	34.5164	-19.9941	-20.6552	-15	-24.6296	28.8378	58.6576	0.0906016	12.726	0.462222	3.81093	
255	0.19509	27.7247	38.2875	21.7882	0	9038.18	42.958	32.8299	28.9558	33.8361	-20.2904	-18.8933	-15	-23.3333	27.7389	57.2648	0.0141621	14.3068	0.465397	4.49787	
256	0.956084	26.5756	38.2875	21.7882	0	9039.18	54.8328	32.3594	31.4011	34.8697	-15.3066	-21.7249	-15	-22.037	26.6577	55.758	0.0821011	0.92513	0.462068	4.62401	
257	0.616135	25.4358	38.2875	21.7882	0	9040.18	60.8887	31.4661	28.4083	33.0811	-12.3747	-22.2226	-15	-20.7407	25.5965	54.125	0.160646	6.76364	0.435175	4.62863	
258	0.896451	24.7463	38.2875	21.7882	0	9041.18	63.5555	30.5469	28.4909	32.3938	-11.0203	-22.157	-15	-19.4444	24.5578	52.3524	0.188505	11.2032	0.403754	4.68469	
259	0.613029	23.3416	38.2875	21.7882	0	9042.18	45.0027	35.1646	32.8384	35.0833	-16.5042	-16.5057	-15	-18.1481	23.5448	50.4252	0.20319	5.42255	0.365921	4.41575	
260	0.28933	22.502	38.2875	21.7882	0	9043.18	46.5666	35.1069	33.1176	35.1511	-15.4704	-16.3404	-15	-16.8519	22.5607	48.3274	0.0587069	1.76077	0.296811	4.4386	
261	1.03413	21.6014	38.2875	21.7882	0	9044.18	38.8167	35.2488	33.7596	35.2221	-16.8309	-13.5404	-15	-15.5556	21.6096	46.0416	0.00817299	7.22493	0.142432	4.40327	
262	1.07655	20.9565	38.2875	21.7882	0	9045.18	37.832	34.9793	33.8497	35.0057	-16.5517	-12.8536	-15	-14.2593	20.696	43.5498	0.260465	5.71781	0.139995	4.11276	
263	0.646108	20.3796	38.2875	21.7882	0	9046.18	43.0291	35.298	35.0902	35.1659	-14.8976	-13.9064	-15	-12.963	19.8252	40.8335	0.554404	2.19564	0.131395	4.05793	
264	1.46053	19.5987	38.2875	21.7882	0	9047.18	52.5753	35.2846	35.0219	35.2042	-11.9105	-15.5643	-15	-11.6667	19.0029	37.875	0.595733	14.7003	0.17308	4.26864	
265	0.767132	18.8763	38.2875	21.7882	0	9048.18	32.1791	35.2687	34.4863	35.2868	-15.9767	-10.0529	-15	-10.3704	18.2358	34.6584	0.640536	2.47922	0.208162	4.44924	
266	0.901855	18.3534	38.2875	21.7882	0	9049.18	30.3363	34.7725	35.135	35.2333	-15.8403	-9.26982	-15	-9.07407	17.5311	31.1713	0.822285	0.835041	0.25753	4.73238	
267	0.829885	17.9312	38.2875	21.7882	0	9050.18	26.7597	35.1186	35.1337	35.1794	-16.0109	-8.07352	-15	-7.77778	16.8966	27.4076	1.03467	0.647923	0.319998	4.98159	
268	0.697108	17.4739	38.2875	21.7882	0	9051.18	20.4336	35.1618	34.02	35.0371	-16.3744	-6.10053	-15	-6.48148	16.3404	23.3691	1.1335	2.93551	0.379238	5.03426	
269	1.46975	16.7821	38.2875	21.7882	0	9052.18	13.4785	35.1603	32.6766	35.1562	-16.3199	-3.91159	-15	-5.18519	15.8709	19.0692	0.911176	5.59065	0.39196	4.67668	
270	0.43712	16.4772	38.2875	21.7882	0	9053.18	12.2806	35.1767	34.7391	35.2455	-16.1002	-3.50469	-15	-3.88889	15.4959	14.5345	0.981306	2.2539	0.395634	4.0517	
271	0.697441	16.1841	38.2876	21.7882	0	9054.18	8.62484	35.1825	35.2087	35.2703	-16.0011	-2.42703	-15	-2.59259	15.2224	9.80609	0.961674	1.18126	0.393012	4.03511	
272	0.544586	15.837	38.2876	21.7882	0	9055.18	2.12198	34.9927	34.4046	35.1065	-15.8261	-0.586398	-15	-1.2963	15.0559	4.93922	0.781081	2.81723	0.379533	4.0215	
273	0.794704	15.3633	38.2876	21.7882	0	9056.18	2.73304	33.2463	33.2436	33.4679	-15.3458	-0.732557	-15	0	15	-0	0.363264	2.73304	0.368216	3.5779	
274	-0.0050352	15.1874	38.2876	21.7882	0	9057.18	1.02278	35.1763	34.8081	35.1267	-15.185	-0.271093	-15	0	15	-0	0.187376	1.02278	0.369517	3.62418	
275	0.821969	15.5438	38.2877	21.7882	0	9058.18	12.8225	35.1003	33.3257	34.7824	-15.1562	-3.44967	-15	0	15	-0	0.543843	12.8225	0.336688	4.28668	
276	0.886725	15.2741	38.2877	21.7882	0	9059.18	9.23176	35.2299	34.9732	35.3306	-15.0763	-2.45041	-15	0	15	-0	0.274147	9.23176	0.305963	4.41249	
277	0.588774	15.3398	38.2877	21.7882	0	9060.18	1.57313	35.1957	34.7299	35.1623	-15.334	-0.421122	-15	0	15	-0	0.339812	1.57313	0.298989	4.45881	
278	0.598484	15.3351	38.2877	21.7882	0	9061.18	-7.06909	35.2544	35.0545	35.2023	-15.2186	1.88723	-15	0	15	-0	0.335121	7.06909	0.310447	4.47973	
279	1.00655	15.2812	38.2877	21.7882	0	9062.18	-0.578342	29.2683	27.9318	27.8786	-15.2804	0.154245	-15	0	15	-0	0.281183	0.578342	0.325389	3.58299	
280	1.2528	15.3304	38.2877	21.7882	0	9063.18	-7.22331	28.1671	27.5665	27.0987	-15.2088	1.9276	-15	0	15	-0	0.330431	7.22331	0.33502	3.68633	
281	0.508385	15.3117	38.2877	21.7883	0	9064.18	-6.82234	35.258	35.0191	35.1521	-15.2033	1.81889	-15	0	15	-0	0.31167	6.82234	0.33878	3.65465	
282	1.4833	15.2906	38.2877	21.7883	0	9065.18	1.58104	35.0553	35.0965	35.2123	-15.2847	-0.42188	-15	0	15	-0	0.290564	1.58104	0.322258	3.5955	
283	0.87971	15.239	38.2877	21.7883	0	9066.18	-4.05548	35.2762	34.9616	35.1308	-15.2008	1.07774	-15	0	15	-0	0.238969	4.05548	0.284119	3.57533	
284	0.715032	15.2835	38.2877	21.7883	0	9067.18	-4.16515	35.2417	34.9737	35.1302	-15.2432	1.11007	-15	0	15	-0	0.283528	4.16515	0.260609	3.56139	
285	1.20328	15.2249	38.2878	21.7883	0	9068.18	-0.279787	35.3054	35.0853	35.2415	-15.2247	0.074346	-15	0	15	-0	0.224899	0.279787	0.216509	3.67861	
286	1.28183	15.2226	38.2878	21.7883	0	9069.18	4.53043	35.328	35.129	35.1814	-15.175	-1.20241	-15	0	15	-0	0.222553	4.53043	0.149039	3.58199	
287	0.574026	15.2014	38.2878	21.7883	0	9070.18	0.73021	35.3225	35.1619	35.0453	-15.2002	-0.193731	-15	0	15	-0	0.201446	0.73021	0.0870744	3.68822	
288	0.951815	15.2038	38.2878	21.7883	0	9071.18	0.0827085	33.0761	32.39	32.5173	-15.2038	-0.0219472	-15	0	15	-0	0.203792	0.0827085	0.0879089	3.82917	
289	0.926552	15.2061	38.2878	21.7883	0	9072.18	1.60918	30.2408	28.3011	29.4855	-15.2001	-0.427015	-15	0	15	-0	0.206137	1.60918	0.0865494	3.79818	
290	0.878243	15.1921	38.2878	21.7883	0	9073.18	1.10396	35.3254	35.2401	35.256	-15.1892	-0.292697	-15	0	15	-0	0.192066	1.10396	0.0526938	3.01236	
291	1.16405	15.2413	38.2878	21.7883	0	9074.18	2.66867	35.331	35.1743	35.3447	-15.2248	-0.709639	-15	0	15	-0	0.241314	2.66867	0.0528536	2.54075	
292	1.12683	15.2812	38.2878	21.7883	0	9075.18	1.05869	35.2833	35.142	35.08	-15.2786	-0.282345	-15	0	15	-0	0.281183	1.05869	0.0485401	2.56386	
293	2.0278	15.3234	38.2878	21.7883	0	9076.18	4.15666	35.2379	35.1774	35.2532	-15.2831	-1.1107	-15	0	15	-0	0.323396	4.15666	0.047258	2.32505	
294	1.0235	15.2953	38.2878	21.7883	0	9077.18	1.1185	35.2703	35.1345	35.0581	-15.2923	-0.298567	-15	0	15	-0	0.295254	1.1185	0.047938	2.29366	
295	1.16544	15.2507	38.2878	21.7883	0	9078.18	1.46956	35.2565	35.1353	35.2243	-15.2457	-0.391116	-15	0	15	-0	0.250695	1.46956	0.0433537	1.94615	
296	0.851286	15.1616	38.2878	21.7883	0	9079.18	-1.54795	35.2859	35.1306	35.2105	-15.156	0.409568	-15	0	15	-0	0.161579	1.54795	0.0456512	1.51044	
297	1.49391	15.1874	38.2878	21.7883	0	9080.18	-0.244302	35.264	35.1111	35.1837	-15.1872	0.0647568	-15	0	15	-0	0.187376	0.244302	0.0454488	1.57562	
298	0.820695	15.1592	38.2878	21.7883	0	9081.18	-2.03685	35.267	35.1358	35.2341	-15.1497	0.538793	-15	0	15	-0	0.159233	2.03685	0.049356	1.46247	
299	0.95971	15.1827	38.2878	21.7883	0	9082.18	0.145993	35.2225	35.1881	35.2423	-15.1826	-0.0386864	-15	0	15	-0	0.182685	0.145993	0.0482484	1.36022	
300	1.35183	15.4078	38.2878	21.7883	0	9083.18	-1.541	35.2137	35.1032	35.2396	-15.4023	0.414351	-15	0	15	-0	0.407822	1.541	0.0680302	1.31643	


==> 06XX/0610/Data/cdf_vld_test_0610_SID8_F5p8GHz_TxG89_RxG75_TD300s_SL9ms.tex <==
0	0.186407	
0.0047619	0.186407	
0.00952381	0.224311	
0.0142857	0.443705	
0.0190476	0.459562	
0.0238095	0.469471	
0.0285714	0.514398	
0.0333333	0.542612	
0.0380952	0.552665	
0.0428571	0.679154	
0.047619	0.686991	
0.052381	0.690065	
0.0571429	0.779046	
0.0619048	0.786002	
0.0666667	0.786963	
0.0714286	0.795093	
0.0761905	0.956428	
0.0809524	0.981667	
0.0857143	1.01299	
0.0904762	1.0152	
0.0952381	1.06968	
0.1	1.1191	
0.104762	1.12464	
0.109524	1.26565	
0.114286	1.29181	
0.119048	1.29224	
0.12381	1.30582	
0.128571	1.32293	
0.133333	1.33706	
0.138095	1.38712	
0.142857	1.53962	
0.147619	1.58307	
0.152381	1.60254	
0.157143	1.6103	
0.161905	1.63022	
0.166667	1.63827	
0.171429	1.67608	
0.17619	1.68089	
0.180952	1.71317	
0.185714	1.91876	
0.190476	1.9429	
0.195238	1.96406	
0.2	1.97924	
0.204762	1.98777	
0.209524	1.9987	
0.214286	2.01785	
0.219048	2.03057	
0.22381	2.0741	
0.228571	2.08107	
0.233333	2.09452	
0.238095	2.1392	
0.242857	2.14152	
0.247619	2.1485	
0.252381	2.1735	
0.257143	2.22043	
0.261905	2.23232	
0.266667	2.24571	
0.271429	2.27633	
0.27619	2.28083	
0.280952	2.29215	
0.285714	2.31725	
0.290476	2.32134	
0.295238	2.32396	
0.3	2.3492	
0.304762	2.36637	
0.309524	2.3766	
0.314286	2.42609	
0.319048	2.43709	
0.32381	2.46369	
0.328571	2.46515	
0.333333	2.49535	
0.338095	2.50308	
0.342857	2.51009	
0.347619	2.51376	
0.352381	2.55826	
0.357143	2.56003	
0.361905	2.56039	
0.366667	2.56273	
0.371429	2.59043	
0.37619	2.61202	
0.380952	2.615	
0.385714	2.61984	
0.390476	2.65553	
0.395238	2.67796	
0.4	2.68865	
0.404762	2.69018	
0.409524	2.70727	
0.414286	2.70953	
0.419048	2.72883	
0.42381	2.748	
0.428571	2.78495	
0.433333	2.79599	
0.438095	2.79623	
0.442857	2.84606	
0.447619	2.8996	
0.452381	2.93578	
0.457143	2.95993	
0.461905	2.98323	
0.466667	3.08288	
0.471429	3.13577	
0.47619	3.32281	
0.480952	3.34571	
0.485714	3.3714	
0.490476	3.41252	
0.495238	3.41608	
0.5	3.47252	
0.504762	3.5224	
0.509524	3.53487	
0.514286	3.71098	
0.519048	3.82538	
0.52381	3.83164	
0.528571	3.85289	
0.533333	3.87402	
0.538095	3.9029	
0.542857	3.99824	
0.547619	4.01205	
0.552381	4.02389	
0.557143	4.05422	
0.561905	4.06024	
0.566667	4.14427	
0.571429	4.17738	
0.57619	4.22324	
0.580952	4.26304	
0.585714	4.26365	
0.590476	4.33917	
0.595238	4.56741	
0.6	4.62184	
0.604762	4.70413	
0.609524	4.79281	
0.614286	4.83861	
0.619048	4.99627	
0.62381	5.03475	
0.628571	5.0608	
0.633333	5.14967	
0.638095	5.25516	
0.642857	5.26338	
0.647619	5.36034	
0.652381	5.42036	
0.657143	5.43515	
0.661905	5.4533	
0.666667	5.50079	
0.671429	5.73296	
0.67619	5.82008	
0.680952	6.06866	
0.685714	6.23535	
0.690476	6.25121	
0.695238	6.25951	
0.7	6.32913	
0.704762	6.36083	
0.709524	6.49319	
0.714286	6.52841	
0.719048	6.72098	
0.72381	6.83072	
0.728571	6.95662	
0.733333	6.98162	
0.738095	7.01047	
0.742857	7.06787	
0.747619	7.13859	
0.752381	7.18892	
0.757143	7.2384	
0.761905	7.28914	
0.766667	7.33587	
0.771429	7.43425	
0.77619	7.46915	
0.780952	7.58644	
0.785714	7.73671	
0.790476	7.78267	
0.795238	7.85319	
0.8	7.86249	
0.804762	7.87168	
0.809524	7.90235	
0.814286	8.03828	
0.819048	8.10024	
0.82381	8.28951	
0.828571	8.3074	
0.833333	8.40967	
0.838095	8.51412	
0.842857	8.55672	
0.847619	8.65286	
0.852381	8.77283	
0.857143	8.85587	
0.861905	9.05069	
0.866667	9.06606	
0.871429	9.11037	
0.87619	9.24354	
0.880952	9.25354	
0.885714	9.31931	
0.890476	9.51146	
0.895238	9.55871	
0.9	9.56168	
0.904762	9.64035	
0.909524	9.74276	
0.914286	10.0934	
0.919048	10.8629	
0.92381	11.3589	
0.928571	11.6184	
0.933333	12.0659	
0.938095	12.1565	
0.942857	12.2003	
0.947619	12.2845	
0.952381	12.4031	
0.957143	12.9209	
0.961905	13.1583	
0.966667	13.4466	
0.971429	13.6717	
0.97619	14.5266	
0.980952	14.7032	
0.985714	16.4664	
0.990476	18.4614	
0.995238	18.5182	
1	26.0323	


==> 06XX/0610/Data/pdf_vld_test_0610_SID8_F5p8GHz_TxG89_RxG75_TD300s_SL9ms.tex <==
0.00111015	0.0619308	
0.0759842	0.330934	
0.123631	0.599936	
0.128212	0.868939	
0.138898	1.13794	
0.157223	1.40694	
0.17435	1.67595	
0.183081	1.94495	
0.181539	2.21395	
0.17187	2.48296	
0.157603	2.75196	
0.141861	3.02096	
0.126722	3.28996	
0.11327	3.55897	
0.101884	3.82797	
0.0925364	4.09697	
0.0850026	4.36597	
0.0789898	4.63498	
0.0742032	4.90398	
0.0703749	5.17298	
0.0672726	5.44198	
0.0647005	5.71099	
0.0624964	5.97999	
0.0605285	6.24899	
0.0586923	6.518	
0.0569076	6.787	
0.0551161	7.056	
0.0532789	7.325	
0.0513735	7.59401	
0.0493915	7.86301	
0.0473353	8.13201	
0.0452163	8.40101	
0.0430514	8.67002	
0.0408613	8.93902	
0.0386684	9.20802	
0.0364948	9.47703	
0.0343613	9.74603	
0.0322864	10.015	
0.0302852	10.284	
0.0283695	10.553	
0.0265476	10.822	
0.0248243	11.091	
0.0232014	11.36	
0.0216779	11.629	
0.0202506	11.898	
0.018915	12.1671	
0.017665	12.4361	
0.0164944	12.7051	
0.0153966	12.9741	
0.0143653	13.2431	
0.0133948	13.5121	
0.0124802	13.7811	
0.0116174	14.0501	
0.0108031	14.3191	
0.0100352	14.5881	
0.00931185	14.8571	
0.00863217	15.1261	
0.00799548	15.3951	
0.00740132	15.6641	
0.00684916	15.9331	
0.00633826	16.2021	
0.00586747	16.4711	
0.00543508	16.7401	
0.00503879	17.0091	
0.00467565	17.2781	
0.0043421	17.5471	
0.0040341	17.8161	
0.00374728	18.0851	
0.00347709	18.3541	
0.00321915	18.6231	
0.00296939	18.8921	
0.00272444	19.1611	
0.00248176	19.4301	
0.00223991	19.6991	
0.00199864	19.9681	
0.00175894	20.2371	
0.00152294	20.5061	
0.00129377	20.7751	
0.00107521	21.0441	
0.000871324	21.3131	
0.000686036	21.5821	
0.000522651	21.8512	
0.000383466	22.1202	
0.000269471	22.3892	
0.000180226	22.6582	
0.000113923	22.9272	
6.76944e-05	23.1962	
3.81508e-05	23.4652	
2.22346e-05	23.7342	
1.86428e-05	24.0032	
3.06181e-05	24.2722	
7.21879e-05	24.5412	
0.000182472	24.8102	
0.00045564	25.0792	
0.00108744	25.3482	
0.00237598	25.6172	
0.00437856	25.8862	
0.00569831	26.1552	
0.00331767	26.4242	
0.000171695	26.6932	


==> 06XX/0610/Data/vld_test_0610_SID8_F5p8GHz_TxG89_RxG75_TD300s_SL9ms.tex <==
1	-0.596857	15.504	38.2879	21.7883	21.7884	78146.2	12.7067	2.50288	5.29168	9.49185	-15.1243	-3.41025	-15	0	15	-0	0.503974	12.7067	NaN	NaN	
2	0.129809	15.4031	38.2879	21.7883	21.7884	78147.2	0.906919	7.89568	12.2428	16.1389	-15.4012	-0.243802	-15	0	15	-0	0.403132	0.906919	NaN	NaN	
3	-0.145469	15.579	38.2879	21.7883	21.7884	78148.2	2.9715	7.18482	11.7557	11.5235	-15.5581	-0.807605	-15	0	15	-0	0.57902	2.9715	NaN	NaN	
4	0.432031	15.5579	38.2879	21.7883	21.7884	78149.2	9.49854	8.02241	10.384	13.1656	-15.3446	-2.56741	-15	0	15	-0	0.557914	9.49854	NaN	NaN	
5	-0.349496	15.6072	38.2879	21.7883	21.7884	78150.2	8.23992	6.29031	8.27734	10.8944	-15.446	-2.2368	-15	0	15	-0	0.607162	8.23992	NaN	NaN	
6	0.126476	15.5907	38.2879	21.7883	21.7884	78151.2	8.40261	2.7911	5.56384	9.28292	-15.4234	-2.27825	-15	0	15	-0	0.590746	8.40261	NaN	NaN	
7	-0.00874634	15.5485	38.2879	21.7883	21.7884	78152.2	0.253078	-6.89278	-4.3115	3.24309	-15.5484	-0.0686783	-15	0	15	-0	0.548533	0.253078	NaN	NaN	
8	-0.0146352	15.5978	38.2879	21.7883	21.7884	78153.2	7.01233	-2.47284	0.290501	5.35785	-15.4811	-1.90422	-15	0	15	-0	0.597782	7.01233	NaN	NaN	
9	0.189531	15.5649	38.2879	21.7883	21.7884	78154.2	10.2394	7.22862	10.7612	13.0464	-15.3171	-2.76684	-15	0	15	-0	0.56495	10.2394	NaN	NaN	
10	0.870147	15.5134	38.2879	21.7883	21.7884	78155.2	9.21161	6.32237	7.79396	13.7561	-15.3133	-2.4834	-15	0	15	-0	0.513355	9.21161	NaN	NaN	
11	-0.20035	15.3726	38.2879	21.7883	21.7884	78156.2	10.0597	-0.843907	3.12156	9.56023	-15.1363	-2.6852	-15	0	15	-0	0.372644	10.0597	NaN	NaN	
12	0.783951	15.4735	38.2878	21.7883	21.7884	78157.2	9.22405	10.0414	13.081	17.7425	-15.2734	-2.48033	-15	0	15	-0	0.473488	9.22405	NaN	NaN	
13	0.442309	15.64	38.2878	21.7883	21.7884	78158.2	4.08543	5.91387	10.4614	16.5542	-15.6003	-1.11425	-15	0	15	-0	0.639995	4.08543	NaN	NaN	
14	-0.0768574	15.5837	38.2878	21.7883	21.7884	78159.2	-4.50908	4.34128	6.31987	13.3909	-15.5355	1.22515	-15	0	15	-0	0.583711	4.50908	NaN	NaN	
15	-0.255746	15.6822	38.2878	21.7883	21.7884	78160.2	9.42969	11.3847	14.8818	19.3348	-15.4703	-2.56933	-15	0	15	-0	0.682209	9.42969	0.0833799	3.69633	
16	0.203837	15.5509	38.2878	21.7883	21.7884	78161.2	5.75835	7.78741	11.2939	11.138	-15.4724	-1.56027	-15	0	15	-0	0.550878	5.75835	0.0824893	3.36642	
17	-0.225837	15.518	38.2878	21.7883	21.7884	78162.2	9.99173	10.6502	12.1873	13.3301	-15.2827	-2.69247	-15	0	15	-0	0.518046	9.99173	0.072504	3.06219	
18	-0.69158	15.6001	38.2878	21.7883	21.7884	78163.2	1.27591	10.2875	12.8856	16.7736	-15.5963	-0.347368	-15	0	15	-0	0.600127	1.27591	0.0731287	3.25687	
19	-0.086163	15.7385	38.2878	21.7883	21.7884	78164.2	8.43128	1.32389	-1.384	5.96677	-15.5684	-2.30763	-15	0	15	-0	0.738492	8.43128	0.0864017	3.21318	
20	-0.00199634	15.9073	38.2878	21.7883	21.7884	78165.2	9.40421	8.9314	11.8138	15.2578	-15.6936	-2.59924	-15	0	15	-0	0.907345	9.40421	0.12237	3.25709	
21	0.0542537	15.7315	38.2878	21.7883	21.7884	78166.2	5.64703	7.97986	11.274	14.1102	-15.6551	-1.54797	-15	0	15	-0	0.731457	5.64703	0.127539	3.25926	
22	0.020841	15.7315	38.2878	21.7883	21.7884	78167.2	10.8034	7.7905	10.5956	15.9024	-15.4526	-2.9487	-15	0	15	-0	0.731457	10.8034	0.130812	2.8145	
23	-0.668802	NaN	38.2878	21.7883	21.7884	78168.2	9.93564	9.80704	11.1312	14.385	NaN	NaN	-15	0	15	-0	NaN	9.93564	0.135673	2.86628	
24	0.681504	15.8862	38.2878	21.7883	21.7884	78169.2	9.16042	6.94768	7.51315	11.6597	-15.6836	-2.52908	-15	0	15	-0	0.886239	9.16042	0.152686	2.81559	
25	-0.873857	15.8886	38.2878	21.7883	21.7884	78170.2	7.23629	8.11893	11.0416	15.256	-15.762	-2.00135	-15	0	15	-0	0.888584	7.23629	0.161818	2.79069	
26	-0.0997867	15.7971	38.2878	21.7883	21.7884	78171.2	6.78169	9.05577	11.229	14.8637	-15.6866	-1.86543	-15	0	15	-0	0.797122	6.78169	0.141379	2.71702	
27	-0.0962592	15.7737	38.2878	21.7883	21.7884	78172.2	6.54395	9.00839	12.0981	16.2766	-15.6709	-1.79765	-15	0	15	-0	0.77367	6.54395	0.127269	2.67953	
28	-0.471969	15.6423	38.2878	21.7883	21.7884	78173.2	2.65084	7.0205	10.4709	16.4907	-15.6256	-0.723449	-15	0	15	-0	0.64234	2.65084	0.127162	2.82294	
29	-0.675413	15.6846	38.2878	21.7883	21.7884	78174.2	2.78944	-3.15499	0.463995	3.20894	-15.666	-0.7633	-15	0	15	-0	0.684553	2.78944	0.121802	2.96984	
30	-0.15658	15.5884	38.2878	21.7883	21.7884	78175.2	8.59621	3.2795	8.89748	9.0917	-15.4133	-2.33	-15	0	15	-0	0.588401	8.59621	0.126743	2.92979	
31	-0.344357	15.5603	38.2878	21.7883	21.7884	78176.2	14.3333	5.81089	5.6472	10.5597	-15.0759	-3.85214	-15	0	15	-0	0.560259	14.3333	0.125818	3.45892	
32	-0.992958	15.6423	38.2878	21.7883	21.7884	78177.2	6.8628	10.1479	13.9159	15.4919	-15.5303	-1.86914	-15	0	15	-0	0.64234	6.8628	0.114523	3.39636	
33	0.35342	15.6775	38.2878	21.7883	21.7884	78178.2	8.75522	10.5072	12.5259	13.6015	-15.4948	-2.38633	-15	0	15	-0	0.677518	8.75522	0.109715	2.95976	
34	-0.262691	15.6588	38.2878	21.7883	21.7884	78179.2	-1.60957	-0.0407244	4.36832	9.41408	-15.6526	0.439834	-15	0	15	-0	0.658756	1.60957	0.111416	3.36272	
35	0.27092	15.701	38.2878	21.7883	21.7884	78180.2	9.41634	10.4367	12.6819	15.6783	-15.4894	-2.56879	-15	0	15	-0	0.700969	9.41634	0.0985479	3.36324	
36	0.243004	15.9965	38.2878	21.7883	21.7884	78181.2	7.57571	1.85782	6.89141	6.24622	-15.8568	-2.10891	-15	0	15	-0	0.996462	7.57571	0.124635	3.32778	
37	0.0645567	16.8149	38.2878	21.7883	21.7884	78182.2	22.5907	-5.27737	-10.8094	1.20878	-15.5248	-6.45939	-16.1864	-0	16.1864	-0	0.628489	22.5907	0.127585	5.08307	
38	-0.0729686	NaN	38.2878	21.7883	21.7884	78183.2	11.3096	3.78653	2.72438	6.24134	NaN	NaN	-17.3729	-0	17.3729	-0	NaN	11.3096	0.127585	5.12641	
39	0.0928648	18.3463	38.2878	21.7883	21.7884	78184.2	10.3817	9.72503	11.3505	12.2316	-18.046	-3.30609	-18.5593	-0	18.5593	-0	0.212991	10.3817	0.178251	5.14876	
40	0.815062	19.4087	38.2878	21.7883	21.7884	78185.2	10.3125	8.43734	8.16054	9.5855	-19.0952	-3.47448	-19.7458	-0	19.7458	-0	0.337066	10.3125	0.188129	5.15628	
41	0.562587	20.8252	38.2878	21.7883	21.7884	78186.2	5.89126	8.79169	10.8744	12.8164	-20.7152	-2.13752	-20.9322	-0	20.9322	-0	0.107019	5.89126	0.228649	5.18499	
42	0.533004	21.7867	38.2878	21.7883	21.7884	78187.2	6.07283	6.79553	8.57568	13.2354	-21.6644	-2.30487	-22.1186	-0	22.1186	-0	0.331937	6.07283	0.231295	5.20001	
43	0.857587	23.0085	38.2878	21.7882	21.7884	78188.2	-0.816672	3.45682	10.3727	12.2598	-23.0062	0.327944	-23.3051	-0	23.3051	-0	0.296539	0.816672	0.23956	5.36897	
44	0.087486	24.2937	38.2878	21.7882	21.7884	78189.2	-1.18685	5.50232	5.95358	8.2565	-24.2885	0.503194	-24.4915	-0	24.4915	-0	0.197822	1.18685	0.25051	5.50469	
45	0.246476	25.4639	38.2878	21.7882	21.7884	78190.2	2.85581	-0.75437	4.17122	3.01874	-25.4323	-1.26868	-25.678	-0	25.678	-0	0.214019	2.85581	0.259642	5.68522	
46	0.931867	26.6788	38.2878	21.7882	21.7884	78191.2	5.46735	-1.39816	-0.694426	3.89309	-26.5574	-2.54191	-26.8644	-0	26.8644	-0	0.185657	5.46735	0.268631	5.43489	
47	0.506198	27.8889	38.2878	21.7882	21.7885	78192.2	5.72032	1.23885	1.14877	3.25494	-27.75	-2.77976	-28.0508	-0	28.0508	-0	0.161985	5.72032	0.271729	5.45104	
48	0.408559	29.0802	38.2878	21.7882	21.7885	78193.2	5.69159	3.56666	3.56085	6.03306	-28.9369	-2.88399	-29.2373	-0	29.2373	-0	0.157076	5.69159	0.267538	5.45125	
49	0.659174	30.3255	38.2878	21.7882	21.7885	78194.2	14.9475	1.40747	4.07849	5.03813	-29.2994	-7.82195	-30.4237	-0	30.4237	-0	0.0982268	14.9475	0.262982	5.5735	
50	0.265047	31.5309	38.2878	21.7881	21.7885	78195.2	-34.001	-5.61467	-3.10776	-3.14826	-26.14	17.6323	-31.6102	-0	31.6102	-0	0.0792455	34.001	0.247648	8.73365	
51	0.890762	33.4094	38.2878	21.7881	21.7885	78196.2	3.32822	-0.409299	-0.0611594	3.82489	-33.3531	-1.93961	-32.7966	-0	32.7966	-0	0.612802	3.32822	0.172947	8.87361	
52	0.390285	NaN	38.2878	21.7881	21.7885	78197.2	59.2006	-4.31037	-4.30066	-4.55811	NaN	NaN	-33.9831	-0	33.9831	-0	NaN	59.2006	0.14187	15.4022	
53	0.107587	35.0815	38.2878	21.7881	21.7885	78198.2	2.15328	2.61406	-3.4663	2.88652	-35.0568	-1.31812	-35.1695	-0	35.1695	-0	0.087967	2.15328	0.141504	15.6037	
54	1.45592	36.1392	38.2879	21.7881	21.7885	78199.2	5.55944	-1.58351	-4.63374	-3.24051	-35.9692	-3.5011	-36.3559	-0	36.3559	-0	0.216733	5.55944	0.141493	15.6713	
55	0.554115	37.1476	38.2879	21.7881	21.7885	78200.2	6.20295	-0.385739	-5.10022	1.61865	-36.9301	-4.01382	-37.5424	-0	37.5424	-0	0.394746	6.20295	0.145926	15.7178	
56	0.566254	38.2733	38.2879	21.7881	21.7885	78201.2	-1.35022	-0.223374	-0.137031	3.58103	-38.2627	0.901858	-38.7288	-0	38.7288	-0	0.455502	1.35022	0.153866	15.8582	
57	0.410504	39.46	38.2879	21.7881	21.7885	78202.2	2.95187	2.78631	-0.411219	8.16519	-39.4076	-2.03208	-39.9153	-0	39.9153	-0	0.455282	2.95187	0.162264	15.938	
58	0.482536	40.656	38.2879	21.788	21.7885	78203.2	3.46282	-0.75737	-4.08677	2.24318	-40.5818	-2.45565	-41.1017	-0	41.1017	-0	0.445681	3.46282	0.169706	15.8423	
59	0.78692	41.7958	38.2879	21.788	21.7885	78204.2	0.202973	3.77582	1.17734	6.61265	-41.7955	-0.148063	-42.2881	-0	42.2881	-0	0.492366	0.202973	0.178275	15.8846	
60	0.665143	43.0504	38.2879	21.788	21.7885	78205.2	1.74917	5.03313	1.75859	5.55489	-43.0304	-1.31407	-43.4746	-0	43.4746	-0	0.424136	1.74917	0.180238	15.9237	
61	0.550018	44.2348	38.2879	21.788	21.7885	78206.2	13.0275	-5.65003	-9.94252	-4.9231	-43.0962	-9.97134	-44.661	-0	44.661	-0	0.426261	13.0275	0.179471	15.8851	
62	0.100066	45.4238	38.2879	21.788	21.7885	78207.2	6.447	2.43867	1.30703	7.88501	-45.1365	-5.10036	-45.8475	-0	45.8475	-0	0.423697	6.447	0.175099	15.8701	
63	0.246198	46.5541	38.2879	21.788	21.7885	78208.2	1.8723	3.4609	-0.197217	5.52474	-46.5293	-1.52102	-47.0339	-0	47.0339	-0	0.479761	1.8723	0.17024	15.9862	
64	0.216476	47.6869	38.2879	21.788	21.7885	78209.2	2.30163	3.93562	2.7283	7.60318	-47.6484	-1.91511	-48.2203	-0	48.2203	-0	0.53348	2.30163	0.15727	16.0642	
65	0.407746	48.8759	38.2879	21.788	21.7885	78210.2	1.37314	2.90424	2.00854	4.40307	-48.8618	-1.17124	-49.4068	-0	49.4068	-0	0.530916	1.37314	0.131819	14.6709	
66	-0.366857	50.0203	38.2879	21.788	21.7885	78211.2	-0.62792	3.56229	2.80839	7.11173	-50.0173	0.548175	-50.5932	0	50.5932	-0	0.572909	0.62792	0.127868	14.741	
67	0.261198	51.1788	38.2879	21.7879	21.7885	78212.2	1.05814	1.09774	0.441049	4.35476	-51.1701	-0.945115	-51.7797	0	51.7797	-0	0.600833	1.05814	0.131382	3.31865	
68	-0.215191	52.4405	38.2879	21.7879	21.7885	78213.2	-1.29959	3.88796	3.65548	6.25163	-52.427	1.18936	-52.9661	0	52.9661	-0	0.525567	1.29959	0.0909358	3.34794	
69	-0.506746	53.7116	38.2879	21.7879	21.7885	78214.2	2.04997	-0.770376	1.51893	6.30059	-53.6772	-1.92132	-54.1525	0	54.1525	-0	0.440921	2.04997	0.0605199	3.30099	
70	-0.311719	54.9944	38.2879	21.7879	21.7885	78215.2	4.49358	-5.3714	-8.10986	-2.01391	-54.8254	-4.30867	-55.339	0	55.339	-0	0.344549	4.49358	0.0666558	3.21327	
71	-0.454881	56.2327	38.2879	21.7879	21.7885	78216.2	1.09772	2.07956	1.90774	5.87454	-56.2224	-1.07729	-56.5254	0	56.5254	-0	0.292735	1.09772	0.0818792	3.2229	
72	0.34896	57.4733	38.2879	21.7879	21.7885	78217.2	2.44113	1.7122	1.7042	4.82096	-57.4211	-2.44795	-57.7119	0	57.7119	-0	0.238577	2.44113	0.100821	3.2254	
73	-0.267969	58.7022	38.2879	21.7879	21.7885	78218.2	2.63352	2.6006	2.09934	5.29811	-58.6402	-2.69721	-58.8983	0	58.8983	-0	0.196144	2.63352	0.120513	3.22218	
74	-0.10035	60.0037	38.2879	21.7878	21.7885	78219.2	0.199597	-5.55938	-5.46735	-1.93337	-60.0034	-0.20903	-60.0847	0	60.0847	-0	0.0810103	0.199597	0.149749	3.22237	
75	-0.402016	61.2326	38.2879	21.7878	21.7885	78220.2	0.641609	3.75789	3.4789	6.8277	-61.2288	-0.68568	-61.2712	0	61.2712	-0	0.0385774	0.641609	0.177243	3.26172	
76	-0.380746	62.3255	38.2879	21.7878	21.7885	78221.2	-1.56861	3.14323	4.04226	6.99616	-62.3021	1.7061	-62.4576	0	62.4576	-0	0.132165	1.56861	0.18791	1.61331	
77	0.278698	63.6919	38.2879	21.7878	21.7885	78222.2	-0.162129	1.02885	0.862578	4.52023	-63.6917	0.180228	-63.6441	0	63.6441	-0	0.0478512	0.162129	0.203523	1.1179	
78	0.127929	65.0412	38.2879	21.7878	21.7885	78223.2	3.57297	3.35275	2.90945	6.13846	-64.9148	-4.05335	-64.8305	0	64.8305	-0	0.210671	3.57297	0.2019	1.22947	
79	-0.201699	66.2888	38.2879	21.7878	21.7885	78224.2	2.65996	3.07566	3.11302	3.7987	-66.2174	-3.07636	-66.0169	0	66.0169	-0	0.271865	2.65996	0.193171	1.24534	
80	-0.0773019	68.0618	38.2879	21.7878	21.7885	78225.2	2.80146	0.820387	0.698231	2.97151	-67.9804	-3.32653	-67.2034	0	67.2034	-0	0.858379	2.80146	0.23492	1.27083	
81	0.080696	68.974	38.2879	21.7877	21.7885	78226.2	3.52334	0.514072	-0.168421	-0.148412	-68.8437	-4.23881	-68.3898	0	68.3898	-0	0.584212	3.52334	0.235794	1.29639	
82	0.0882814	69.8676	38.2879	21.7877	21.7885	78227.2	-0.593771	-3.07224	-3.05111	-1.85765	-69.8638	0.724042	-69.5763	0	69.5763	-0	0.291285	0.593771	0.223062	1.32604	
83	0.179254	71.1246	38.2879	21.7877	21.7885	78228.2	-2.0491	-7.57732	-7.61911	-5.6526	-71.0791	2.54312	-70.7627	0	70.7627	-0	0.36186	2.0491	0.215298	1.31251	
84	-0.432302	71.7625	38.2879	21.7877	21.7885	78229.2	-2.2248	1.6632	1.55526	4.38324	-71.7084	2.78585	-71.9492	0	71.9492	-0	0.186693	2.2248	0.21279	1.31346	
85	-0.0948574	74.253	38.2879	21.7877	21.7885	78230.2	-0.901502	0.02844	0.558679	2.35945	-74.2438	1.16826	-73.1356	0	73.1356	-0	1.11745	0.901502	0.304464	1.15259	
86	0.421223	75.2662	38.2879	21.7877	21.7885	78231.2	-1.37721	2.4278	2.77665	4.9765	-75.2444	1.80898	-74.322	0	74.322	-0	0.944123	1.37721	0.343175	1.14256	
87	-0.43008	75.8384	38.2879	21.7877	21.7885	78232.2	5.43938	4.43405	4.06498	7.50758	-75.4969	-7.18891	-75.5085	0	75.5085	-0	0.329905	5.43938	0.341469	1.47287	
88	-0.233246	76.4106	38.2879	21.7877	21.7885	78233.2	2.5905	2.35731	2.15098	3.75966	-76.3325	-3.45356	-76.6949	0	76.6949	-0	0.284311	2.5905	0.338886	1.47164	
89	0.0158608	77.0204	38.2879	21.7876	21.7885	78234.2	-1.74721	-0.0863466	1.48091	2.95063	-76.9845	2.34834	-77.8814	0	77.8814	-0	0.861006	1.74721	0.348981	1.38666	
90	0.184031	78.4837	38.2879	21.7876	21.7885	78235.2	3.63782	-2.00128	-1.70901	-0.768027	-78.3256	-4.97974	-79.0678	0	79.0678	-0	0.584055	3.63782	0.332801	1.37368	
91	-0.105191	79.4359	38.2879	21.7876	21.7885	78236.2	2.34711	0.429495	1.11351	2.95653	-79.3692	-3.25317	-80.2542	0	80.2542	-0	0.818353	2.34711	0.33004	1.35774	
92	-0.203268	NaN	38.2879	21.7876	21.7885	78237.2	0.14317	-1.18205	-0.14667	1.75917	NaN	NaN	-81.4407	0	81.4407	-0	NaN	0.14317	0.31493	1.35996	
93	-0.211302	NaN	38.2879	21.7876	21.7885	78238.2	-0.679813	-3.27743	-2.37863	-0.464283	NaN	NaN	-82.6271	0	82.6271	-0	NaN	0.679813	0.3116	1.38273	
94	0.664476	NaN	38.2879	21.7876	21.7885	78239.2	4.97937	-8.3907	-5.55409	-4.34969	NaN	NaN	-83.8136	0	83.8136	-0	NaN	4.97937	0.311105	1.55861	
95	-0.0673703	NaN	38.2879	21.7876	21.7885	78240.2	-0.568152	0.536662	1.22967	3.62555	NaN	NaN	-85	0	85	-0	NaN	0.568152	0.315092	1.61653	
96	-0.40958	NaN	38.2879	21.7875	21.7885	78241.2	0.0992015	-1.74192	-1.55516	0.772222	NaN	NaN	-85	0	85	-0	NaN	0.0992015	0.33213	1.65561	
97	-0.29808	NaN	38.2879	21.7875	21.7885	78242.2	2.81795	-0.0173191	1.38252	2.44101	NaN	NaN	-85	0	85	-0	NaN	2.81795	0.335693	1.62395	
98	-0.641746	NaN	38.2879	21.7875	21.7885	78243.2	4.1007	-6.83188	-6.7952	-2.99453	NaN	NaN	-85	0	85	-0	NaN	4.1007	0.344837	1.7032	
99	-0.29908	NaN	38.2879	21.7875	21.7885	78244.2	1.7785	-0.514505	-0.355921	3.33552	NaN	NaN	-85	0	85	-0	NaN	1.7785	0.315378	1.70745	
100	0.0428395	86.5324	38.2879	21.7875	21.7885	78245.2	-0.0995617	-1.85586	-2.34144	1.14354	-86.5323	0.150365	-85	0	85	-0	1.53239	0.0995617	0.425471	1.76312	
101	0.63792	NaN	38.2879	21.7875	21.7885	78246.2	2.09315	-0.0891776	-0.659179	2.12654	NaN	NaN	-85	0	85	-0	NaN	2.09315	0.457967	1.75005	
102	-0.0895645	NaN	38.2879	21.7875	21.7885	78247.2	-0.630413	-2.05715	-2.25105	1.31735	NaN	NaN	-85	0	85	-0	NaN	0.630413	0.46145	1.54419	
103	-0.399996	NaN	38.2879	21.7875	21.7885	78248.2	-3.24751	-4.95585	-4.97111	-1.80424	NaN	NaN	-85	0	85	-0	NaN	3.24751	0.407572	1.57458	
104	0.311728	NaN	38.2879	21.7875	21.7885	78249.2	-0.591012	-3.50417	-3.3989	-0.230762	NaN	NaN	-85	0	85	-0	NaN	0.591012	0.49398	1.61209	
105	0.126476	NaN	38.2879	21.7875	21.7885	78250.2	0.770342	-4.58072	-4.01004	-0.720057	NaN	NaN	-85	0	85	-0	NaN	0.770342	0.504903	1.55446	
106	0.00425366	NaN	38.2879	21.7875	21.7885	78251.2	3.15553	-2.91137	-4.04547	0.119647	NaN	NaN	-85	0	85	-0	NaN	3.15553	0	1.5934	
107	-0.112573	NaN	38.2879	21.7875	21.7885	78252.2	-1.19459	-1.78692	-2.19397	0.933522	NaN	NaN	-85	0	85	-0	NaN	1.19459	0	1.5415	
108	0.158698	NaN	38.2879	21.7875	21.7885	78253.2	-1.30345	-0.841598	-1.42402	1.83899	NaN	NaN	-85	0	85	-0	NaN	1.30345	0	1.51773	
109	-0.12908	NaN	38.2879	21.7876	21.7885	78254.2	-1.15563	-1.146	-1.85771	1.53697	NaN	NaN	-85	0	85	-0	NaN	1.15563	0	1.24786	
110	0.195754	NaN	38.2879	21.7875	21.7885	78255.2	0.411416	-1.67375	-2.52875	0.432847	NaN	NaN	-85	0	85	-0	NaN	0.411416	0	1.2575	
111	-0.254635	NaN	38.2879	21.7875	21.7885	78256.2	3.13226	-2.72128	-3.45964	-0.425775	NaN	NaN	-85	0	85	-0	NaN	3.13226	0	1.24909	
112	-0.774635	NaN	38.2879	21.7875	21.7885	78257.2	1.62775	-0.865807	-0.536086	2.82722	NaN	NaN	-85	0	85	-0	NaN	1.62775	0	1.21479	
113	-0.649592	NaN	38.2879	21.7875	21.7885	78258.2	1.33886	-0.0855219	0.0678618	3.17463	NaN	NaN	-85	0	85	-0	NaN	1.33886	0	1.01566	
114	-1.33138	NaN	38.2879	21.7876	21.7885	78259.2	7.40633	-2.64868	-2.30856	1.918	NaN	NaN	-85	0	85	-0	NaN	7.40633	0	1.8345	
115	NaN	NaN	38.2879	21.7876	21.7885	78260.2	-2.11641	-1.86248	-2.40115	1.28835	NaN	NaN	-85	0	85	-0	NaN	2.11641	NaN	1.76759	
116	-1.87775	85.538	38.2879	21.7876	21.7885	78261.2	0.385016	-0.650953	-0.624675	2.9494	-85.5361	-0.574794	-85	0	85	-0	0.538038	0.385016	0	1.81632	
117	-1.05432	NaN	38.2879	21.7876	21.7885	78262.2	0.0446761	-0.538789	-0.356599	3.24696	NaN	NaN	-83.75	-0	83.75	-0	NaN	0.0446761	0	1.85147	
118	-0.706996	NaN	38.2879	21.7876	21.7885	78263.2	2.37433	-0.881446	-0.976836	2.60871	NaN	NaN	-82.5	0	82.5	-0	NaN	2.37433	0	1.81811	
119	-1.02829	81.2557	38.2879	21.7876	21.7885	78264.2	2.08732	-0.241096	-0.733403	2.77437	-81.2018	-2.95954	-81.25	0	81.25	-0	0.005742	2.08732	0.37639	1.7878	
120	-1.17225	NaN	38.2879	21.7876	21.7885	78265.2	0.873079	1.13882	1.00728	4.81404	NaN	NaN	-80	0	80	-0	NaN	0.873079	0.37639	1.78336	
121	-0.912096	NaN	38.2879	21.7876	21.7885	78266.2	5.92875	0.665306	0.434112	4.95326	NaN	NaN	-80	0	80	-0	NaN	5.92875	0.37639	2.04638	
122	-1.83716	NaN	38.2879	21.7876	21.7885	78267.2	3.49521	0.584739	0.262462	4.72928	NaN	NaN	-80	0	80	-0	NaN	3.49521	0.37639	2.06048	
123	-1.77563	NaN	38.2879	21.7876	21.7885	78268.2	3.62982	0.0471335	-0.245311	4.06545	NaN	NaN	-80	0	80	-0	NaN	3.62982	0.37639	2.07204	
124	-1.43219	NaN	38.2879	21.7876	21.7885	78269.2	4.45895	-0.107448	-0.168974	4.5124	NaN	NaN	-80	0	80	-0	NaN	4.45895	0.37639	2.10556	
125	-1.44169	NaN	38.2879	21.7876	21.7885	78270.2	2.21497	-0.435269	0.138105	4.06308	NaN	NaN	-80	0	80	-0	NaN	2.21497	0.37639	2.02015	
126	-1.01441	NaN	38.2879	21.7876	21.7885	78271.2	2.77209	-0.714746	-0.554655	3.48906	NaN	NaN	-80	0	80	-0	NaN	2.77209	0.37639	2.01731	
127	-1.15686	NaN	38.2879	21.7876	21.7885	78272.2	6.20966	-0.0953719	-0.0684947	4.03069	NaN	NaN	-80	0	80	-0	NaN	6.20966	0.37639	2.18087	
128	-1.70852	NaN	38.2879	21.7876	21.7885	78273.2	3.34253	-1.28851	-1.41794	2.67645	NaN	NaN	-80	0	80	-0	NaN	3.34253	0.37639	2.13119	
129	-1.8438	NaN	38.2879	21.7876	21.7885	78274.2	5.36522	-0.256223	-0.207041	4.2294	NaN	NaN	-80	0	80	-0	NaN	5.36522	0.37639	1.89218	
130	-1.23746	NaN	38.2879	21.7876	21.7885	78275.2	1.7011	-5.33798	-5.28184	-1.11223	NaN	NaN	-80	0	80	-0	NaN	1.7011	0.37639	1.90931	
131	-0.880393	NaN	38.2879	21.7876	21.7885	78276.2	2.43181	-1.01972	-0.724171	3.09983	NaN	NaN	-80	0	80	-0	NaN	2.43181	0	1.77832	
132	-1.03477	NaN	38.2879	21.7876	21.7885	78277.2	2.47172	-2.0404	-1.7742	2.29842	NaN	NaN	-80	0	80	-0	NaN	2.47172	0	1.57665	
133	-0.923969	NaN	38.2879	21.7876	21.7885	78278.2	2.57205	-3.20187	-2.55073	1.47462	NaN	NaN	-80	0	80	-0	NaN	2.57205	0	1.56926	
134	-0.972584	NaN	38.2879	21.7876	21.7885	78279.2	2.95591	-3.13415	-2.50376	0.666333	NaN	NaN	-80	0	80	-0	NaN	2.95591	NaN	1.53686	
135	-1.32339	NaN	38.2879	21.7876	21.7885	78280.2	2.07983	-0.927364	-1.24801	1.86918	NaN	NaN	-80	0	80	-0	NaN	2.07983	NaN	1.42479	
136	-0.595746	80.5334	38.2879	21.7876	21.7885	78281.2	3.90883	1.25786	1.24709	5.56889	-80.3461	-5.48989	-80	0	80	-0	0.533427	3.90883	0	1.25875	
137	-1.73019	80.6413	38.2879	21.7876	21.7885	78282.2	5.50205	2.32378	0.300885	6.05784	-80.2698	-7.732	-80	0	80	-0	0.641306	5.50205	0.076282	1.38088	
138	-1.74658	80.6835	38.2878	21.7876	21.7885	78283.2	1.50666	-2.53932	2.20335	3.85575	-80.6556	-2.12143	-80	0	80	-0	0.683519	1.50666	0.0774031	1.46632	
139	-0.257969	80.8993	38.2878	21.7876	21.7885	78284.2	6.03267	-0.194994	4.24095	6.36683	-80.4513	-8.50215	-80	0	80	-0	0.899276	6.03267	0.153539	1.60495	
140	-0.953385	80.9931	38.2878	21.7876	21.7885	78285.2	4.90245	-1.27715	-0.617451	2.95693	-80.6968	-6.92163	-80	0	80	-0	0.993082	4.90245	0.190072	1.61266	
141	-1.49019	81.0892	38.2878	21.7876	21.7885	78286.2	8.23566	-1.01357	0.512049	3.63724	-80.253	-11.6156	-80	0	80	-0	1.08924	8.23566	0.219245	1.9893	
142	-1.25908	81.2276	38.2878	21.7876	21.7885	78287.2	11.1121	1.54242	3.74037	7.44482	-79.7047	-15.6549	-80	-2.5	80.0391	1.78991	1.18855	9.3222	0.246765	2.3683	
143	-0.828524	81.2933	38.2878	21.7876	21.7885	78288.2	10.1452	1.94954	3.69703	6.83397	-80.0222	-14.3193	-80	-5	80.1561	3.57633	1.13717	6.56888	0.248423	2.43478	
144	-1.505	81.4762	38.2878	21.7876	21.7885	78289.2	18.4735	-4.16971	-3.94133	-2.2932	-77.2778	-25.817	-80	-7.5	80.3508	5.35583	1.1254	13.1176	0.244667	3.32212	
145	-1.79575	NaN	38.2878	21.7876	21.7885	78290.2	13.0375	-0.398003	0.839404	2.99585	NaN	NaN	-80	-10	80.6226	7.12502	NaN	5.91252	0.244667	3.20967	
146	-1.75219	81.9405	38.2878	21.7876	21.7885	78291.2	12.2156	0.124102	2.6189	5.38	-80.0853	-17.3379	-80	-12.5	80.9707	8.88066	0.96986	3.33493	0.231187	3.16281	
147	-0.912191	NaN	38.2877	21.7876	21.7885	78292.2	16.439	2.60194	1.23451	5.92801	NaN	NaN	-80	-15	81.3941	10.6197	NaN	5.81938	0.231187	3.07119	
148	-1.49352	82.5174	38.2877	21.7876	21.7885	78293.2	11.2838	1.00891	1.33208	5.27664	-80.9224	-16.1461	-80	-17.5	81.8917	12.3391	0.625751	1.0553	0.237281	3.19522	
149	-1.55575	NaN	38.2877	21.7876	21.7885	78294.2	16.8331	-7.3455	-7.33337	-2.51364	NaN	NaN	-80	-20	82.4621	14.0362	NaN	2.79681	0.237281	3.20399	
150	-1.24166	NaN	38.2877	21.7876	21.7885	78295.2	12.3939	-10.9941	-9.90249	-6.17567	NaN	NaN	-80	-22.5	83.1039	15.7086	NaN	3.31473	0.237281	3.12924	
151	-0.862524	NaN	38.2877	21.7876	21.7885	78296.2	31.9112	-21.2692	-21.7129	-17.0833	NaN	NaN	-80	-25	83.8153	17.354	NaN	14.5572	0.215044	3.87936	
152	-1.60144	NaN	38.2877	21.7876	21.7885	78297.2	19.4378	-11.0313	-12.3472	-7.07517	NaN	NaN	-80	-27.5	84.5946	18.9704	NaN	0.46737	0.200047	4.14636	
153	-1.52544	NaN	38.2877	21.7876	21.7885	78298.2	17.8595	-11.7911	-14.2451	-6.52534	NaN	NaN	-80	-30	85.44	20.556	NaN	2.69651	0.180916	4.0691	
154	-0.931302	NaN	38.2877	21.7876	21.7885	78299.2	25.9774	-6.34133	-7.38995	-3.54081	NaN	NaN	-80	-32.5	86.3496	22.1094	NaN	3.86795	0.19004	4.10139	
155	-1.61575	NaN	38.2876	21.7876	21.7885	78300.2	23.2428	-6.89454	-6.13144	-4.16662	NaN	NaN	-80	-35	87.3212	23.6294	NaN	0.38659	0.207818	4.32616	
156	-1.51825	NaN	38.2876	21.7876	21.7885	78301.2	17.7906	-9.17778	-7.2643	-1.60116	NaN	NaN	-80	-35	87.3212	23.6294	NaN	5.83882	0.229468	4.25888	
157	-0.312157	NaN	38.2876	21.7876	21.7885	78302.2	25.2099	-9.78002	-5.88179	-4.34419	NaN	NaN	-80	-35	87.3212	23.6294	NaN	1.58048	0.238384	4.2015	
158	-1.11565	NaN	38.2876	21.7876	21.7885	78303.2	21.187	-1.00121	0.0324564	5.92138	NaN	NaN	-80	-35	87.3212	23.6294	NaN	2.44241	0.255684	4.20929	
159	-1.10866	85.9133	38.2876	21.7876	21.7885	78304.2	21.0508	-5.4037	-6.52034	0.957613	-80.1796	-30.8596	-80	-35	87.3212	23.6294	1.40798	2.5786	0.392054	3.48096	
160	-1.1416	NaN	38.2876	21.7876	21.7885	78305.2	28.0156	-1.66327	-7.38456	0.923625	NaN	NaN	-80	-35	87.3212	23.6294	NaN	4.38627	0.392054	3.43609	
161	-1.10447	NaN	38.2876	21.7876	21.7885	78306.2	18.1291	-11.1086	-7.3377	-5.77778	NaN	NaN	-80	-35	87.3212	23.6294	NaN	5.50028	0.553119	3.46614	
162	-1.15494	NaN	38.2876	21.7876	21.7885	78307.2	23.2315	-2.11624	-5.30164	-0.173227	NaN	NaN	-80	-35	87.3212	23.6294	NaN	0.397893	0.553119	3.52484	
163	-0.936746	NaN	38.2876	21.7876	21.7885	78308.2	28.3417	-8.02107	-8.98158	-5.3983	NaN	NaN	-80	-35	87.3212	23.6294	NaN	4.71231	0	3.47289	
164	-1.46301	87.5901	38.2876	21.7876	21.7885	78309.2	17.3128	-6.03397	-7.3217	-3.72858	-83.6217	-26.0658	-80	-35	87.3212	23.6294	0.268824	6.31654	0.805505	3.52589	
165	-0.454029	87.644	38.2875	21.7876	21.7885	78310.2	26.4141	-8.11174	-11.1569	-4.99538	-78.4942	-38.9889	-80	-35	87.3212	23.6294	0.322762	2.7847	0.642687	3.53521	
166	-1.98464	87.6252	38.2875	21.7876	21.7885	78311.2	21.001	-10.3602	-12.6728	-8.68855	-81.8047	-31.4035	-80	-35	87.3212	23.6294	0.304001	2.62838	0.555175	1.95566	
167	-0.77815	NaN	38.2875	21.7876	21.7885	78312.2	25.2721	-7.77424	-9.76832	-5.04032	NaN	NaN	-80	-35	87.3212	23.6294	NaN	1.64271	0.555175	1.86379	
168	-0.794208	87.6182	38.2876	21.7876	21.7885	78313.2	24.0295	-5.29667	-7.30342	-3.43981	-80.0249	-35.6787	-80	-35	87.3212	23.6294	0.296966	0.400089	0.496714	1.9963	
169	-1.3308	87.6299	38.2876	21.7876	21.7885	78314.2	23.4064	-5.47504	-6.93477	-2.60957	-80.4189	-34.811	-80	-35	87.3212	23.6294	0.308692	0.222993	0.452581	2.10597	
170	-0.85211	87.6581	38.2875	21.7876	21.7885	78315.2	27.1334	-6.78419	-9.66912	-4.8603	-78.011	-39.9777	-80	-35	87.3212	23.6294	0.336834	3.50403	0.416919	2.00338	
171	-1.07352	87.6276	38.2875	21.7876	21.7885	78316.2	26.1781	-5.94801	-8.22208	-4.79399	-78.6394	-38.6581	-80	-35	87.3212	23.6294	0.306347	2.54873	0.389982	1.84362	
172	-0.518575	87.6041	38.2876	21.7876	21.7885	78317.2	24.98	-5.11461	-9.15391	-4.59565	-79.4092	-36.9954	-80	-35	87.3212	23.6294	0.282895	1.35066	0.368729	1.85519	
173	-0.484592	87.5901	38.2876	21.7876	21.7885	78318.2	32.1003	-5.08557	-9.421	-5.26571	-74.1992	-46.5456	-80	-35	87.3212	23.6294	0.268823	8.4709	0.351182	2.36434	
174	-0.827642	87.6464	38.2876	21.7876	21.7885	78319.2	34.4276	-6.5028	-9.79869	-5.89982	-72.2943	-49.5522	-80	-35	87.3212	23.6294	0.325108	10.7982	0.0231845	3.06725	
175	-0.902099	87.5666	38.2876	21.7876	21.7885	78320.2	29.6867	-8.196	-11.7688	-7.9141	-76.0732	-43.368	-80	-35	87.3212	23.6294	0.245372	6.05733	0.0278672	3.12336	
176	-1.07936	NaN	38.2876	21.7876	21.7885	78321.2	26.195	-3.49792	-7.56025	-1.20146	NaN	NaN	-80	-35	87.3212	23.6294	NaN	2.56561	0.0278672	3.1026	
177	-0.545746	NaN	38.2876	21.7876	21.7885	78322.2	19.9252	-6.19874	-6.58683	-2.70858	NaN	NaN	-78.6735	-35	86.1076	23.9832	NaN	4.05793	0.0278672	2.97169	
178	-0.986746	87.5455	38.2876	21.7876	21.7885	78323.2	20.7175	-2.34461	-5.88676	0.911967	-81.8845	-30.9702	-77.3469	-35	84.8973	24.3471	2.64823	3.62955	0.67927	2.96292	
179	-0.841937	86.9334	38.2876	21.7876	21.7885	78324.2	26.4904	-5.07515	-9.43889	-4.53527	-77.8062	-38.7764	-76.0204	-35	83.6905	24.7215	3.2429	1.7689	1.03795	2.91921	
180	-0.223969	86.1853	38.2876	21.7876	21.7885	78325.2	24.4413	-1.70191	-6.32837	0.188269	-78.4619	-35.6601	-74.6939	-35	82.4874	25.1068	3.69788	0.665532	1.33046	3.00605	
181	-1.28892	84.9306	38.2876	21.7876	21.7885	78326.2	22.373	-1.74011	-3.02828	1.84483	-78.5375	-32.3275	-73.3673	-35	81.2882	25.5035	3.64246	3.13058	1.50435	3.00018	
182	-0.731496	NaN	38.2876	21.7876	21.7885	78327.2	23.8959	-5.20131	-10.0453	-2.70726	NaN	NaN	-72.0408	-35	80.0929	25.9121	NaN	2.01625	1.50435	2.98618	
183	0.057587	NaN	38.2876	21.7876	21.7885	78328.2	8.29895	-15.2891	-13.7471	-11.2135	NaN	NaN	-70.7143	-35	78.9019	26.3331	NaN	18.0341	1.54259	4.69673	
184	-0.44908	NaN	38.2876	21.7876	21.7885	78329.2	20.1335	-4.8227	-5.68307	-0.319909	NaN	NaN	-69.3878	-35	77.7153	26.7669	NaN	6.63339	1.58136	4.56085	
185	-0.28208	NaN	38.2876	21.7877	21.7885	78330.2	20.4916	-5.34195	-7.31485	-0.734616	NaN	NaN	-68.0612	-35	76.5332	27.2142	NaN	6.72256	1.62033	4.56038	
186	0.0162729	NaN	38.2876	21.7877	21.7885	78331.2	32.101	-14.265	-14.0347	-5.4313	NaN	NaN	-66.7347	-35	75.356	27.6754	NaN	4.42553	1.64907	4.50699	
187	0.178869	NaN	38.2876	21.7877	21.7885	78332.2	22.0828	-7.97098	-8.33431	-3.8898	NaN	NaN	-65.4082	-35	74.1837	28.1513	NaN	6.06851	1.65458	4.37011	
188	-0.0567781	NaN	38.2876	21.7877	21.7885	78333.2	27.0108	-5.91825	-8.87697	-3.85714	NaN	NaN	-64.0816	-35	73.0168	28.6424	NaN	1.63158	1.60551	4.41355	
189	-0.00104548	NaN	38.2876	21.7877	21.7885	78334.2	32.6565	-4.63432	-5.90797	-2.06986	NaN	NaN	-62.7551	-35	71.8554	29.1494	NaN	3.50706	1.43235	4.14809	
190	0.590476	NaN	38.2876	21.7877	21.7885	78335.2	17.7744	-11.1173	-12.2005	-5.36655	NaN	NaN	-61.4286	-35	70.6999	29.6731	NaN	11.8987	0.484221	4.53773	
191	-0.23035	73.9716	38.2876	21.7877	21.7885	78336.2	25.0099	-12.4593	-18.8726	-6.45958	-67.0357	-31.2733	-60.102	-35	69.5504	30.2141	4.42124	5.20421	0.650977	4.48257	
192	-0.129318	72.8553	38.2876	21.7878	21.7885	78337.2	21.3659	-11.3365	-11.0528	-4.56757	-67.8482	-26.5428	-58.7755	-35	68.4073	30.7732	4.448	9.40734	0.692319	4.58883	
193	-0.862312	71.7085	38.2876	21.7878	21.7885	78338.2	19.9216	-9.75601	-11.9335	-4.61359	-67.4175	-24.4335	-57.449	-35	67.271	31.3513	4.43754	11.4297	0.521512	4.78148	
194	-0.413663	70.5383	38.2876	21.7878	21.7885	78339.2	26.4793	-6.81865	-10.8671	-1.78601	-63.1385	-31.4512	-56.1224	-35	66.1417	31.9492	4.39654	5.46987	0.390999	4.63131	
195	-0.496302	69.3751	38.2876	21.7878	21.7885	78340.2	25.7372	-5.92242	-7.89758	-4.11651	-62.4927	-30.1258	-54.7959	-35	65.0199	32.5677	4.35513	6.8305	0.315785	4.34948	
196	0.416274	68.3596	38.2876	21.7878	21.7885	78341.2	10.8322	-15.7275	-18.6831	-10.5685	-67.1416	-12.8471	-53.4694	-35	63.906	33.208	4.45362	22.3757	0.0373401	5.78328	
197	0.26592	67.2198	38.2876	21.7878	21.7885	78342.2	45.2988	-6.38497	-7.75063	-6.59714	-47.2831	-47.7788	-52.1429	-35	62.8003	33.8708	4.41955	11.428	0.0340883	5.58193	
198	-0.200105	65.8057	38.2876	21.7878	21.7885	78343.2	31.3263	-4.80317	-7.31496	-3.09609	-56.2126	-34.2131	-50.8163	-35	61.7033	34.5573	4.10239	3.23101	0.116234	5.10955	
199	0.109296	64.9779	38.2876	21.7878	21.7885	78344.2	24.9843	-12.8251	-12.1152	-6.83907	-58.8974	-27.4447	-49.4898	-35	60.6155	35.2686	4.36235	10.2842	0.108873	5.13938	
200	0.113837	63.9085	38.2876	21.7879	21.7885	78345.2	30.5856	-12.6967	-12.9377	-10.0001	-55.0169	-32.5182	-48.1633	-35	59.5374	36.0057	4.37107	5.42015	0.102666	5.17329	
201	-0.191857	62.9774	38.2876	21.7879	21.7885	78346.2	35.807	-12.9088	-10.8588	-8.59763	-51.0742	-36.8454	-46.8367	-35	58.4695	36.7699	4.50795	0.962857	0.105124	5.41153	
202	-0.371937	61.8799	38.2876	21.7879	21.7885	78347.2	34.6115	-8.01689	-2.86017	3.10059	-50.9285	-35.1483	-45.5102	-35	57.4124	37.5624	4.46752	2.9509	0.102784	5.53614	
203	0.464961	60.3461	38.2876	21.7879	21.7885	78348.2	38.0046	-11.4083	-7.27345	-3.86348	-47.5504	-37.1566	-44.1837	-35	56.3666	38.3844	3.9795	0.379797	0.15159	5.6389	
204	0.211143	59.2509	38.2876	21.7879	21.7885	78349.2	34.0101	0.193122	-4.23238	0.118214	-49.1154	-33.1414	-42.8571	-35	55.3329	39.2374	3.91799	5.22724	0.188079	5.57148	
205	-0.163019	58.1604	38.2876	21.7879	21.7885	78350.2	37.2101	-0.882059	-3.0602	1.31275	-46.3203	-35.1719	-41.5306	-35	54.312	40.1226	3.84844	2.9125	0.220002	5.5478	
206	-0.0954849	57.0676	38.2876	21.7879	21.7885	78351.2	40.2919	-5.11629	-5.11788	-0.742224	-43.5288	-36.9046	-40.2041	-35	53.3045	41.0415	3.76309	0.749574	0.256533	5.76027	
207	-0.123524	55.8528	38.2876	21.788	21.7885	78352.2	26.8248	-15.324	-10.1929	-4.95164	-49.8425	-25.2044	-38.8776	-35	52.3112	41.9955	3.54155	15.1707	0.309262	6.1403	
208	0.370578	54.8537	38.2876	21.788	21.7885	78353.2	35.9118	-5.0231	-0.620131	2.56431	-44.4272	-32.1739	-37.551	-35	51.333	42.9862	3.5207	7.07437	0.346279	6.01701	
209	1.39842	53.7515	38.2876	21.788	21.7885	78354.2	31.1301	-9.68644	-8.48449	-0.956959	-46.011	-27.7886	-36.2245	-35	50.3708	44.0151	3.38073	12.885	0.388042	6.21041	
210	1.20303	52.607	38.2876	21.788	21.7885	78355.2	31.721	-13.0849	-8.32355	-2.83528	-44.7485	-27.6599	-34.898	-35	49.4254	45.0836	3.18167	13.3626	0.44037	6.40908	
211	-0.113019	51.5822	38.2876	21.788	21.7885	78356.2	36.6729	-5.67386	-6.4913	-2.33654	-41.3719	-30.8073	-33.5714	-35	48.4978	46.1935	3.08436	9.52056	0.477299	5.00091	
212	0.32587	50.5316	38.2876	21.788	21.7885	78357.2	42.6269	-3.46667	-1.88016	2.13768	-37.1801	-34.2211	-32.2449	-35	47.5892	47.3462	2.94234	4.71927	0.512767	4.85242	
213	0.801754	49.4551	38.2876	21.7881	21.7885	78358.2	40.6854	-7.91842	-3.92305	-1.21983	-37.5018	-32.2401	-30.9184	-35	46.7006	48.5432	2.75453	7.8578	0.570487	4.78844	
214	0.524254	48.7703	38.2876	21.7881	21.7885	78359.2	40.9511	-7.79646	-8.82485	-2.07641	-36.8348	-31.9648	-29.5918	-35	45.8331	49.7861	2.93719	8.83506	0.572442	4.72367	
215	0.940851	NaN	38.2876	21.7881	21.7885	78360.2	42.7337	-4.49701	-1.86144	3.48191	NaN	NaN	-28.2653	-35	44.9881	51.0763	NaN	8.34263	0.552778	4.73465	
216	0.737587	47.2319	38.2876	21.7881	21.7885	78361.2	54.0246	-11.0815	-9.35376	-4.49578	-27.7458	-38.2233	-26.9388	-35	44.1667	52.4153	3.06519	1.60934	0.493599	4.68104	
217	0.603857	45.6512	38.2876	21.7881	21.7885	78362.2	38.3243	-1.93384	-0.298528	4.95522	-35.814	-28.3089	-25.6122	-35	43.3703	53.8041	2.2809	15.4798	0.494877	5.0533	
218	0.570047	44.7249	38.2876	21.7881	21.7885	78363.2	42.9875	0.473735	-2.26257	4.39268	-32.7164	-30.4952	-24.2857	-35	42.6004	55.2441	2.12448	12.2565	0.544737	4.76183	
219	1.12183	NaN	38.2876	21.7881	21.7885	78364.2	53.6132	-1.87173	-6.29253	-1.84315	NaN	NaN	-22.9592	-35	41.8584	56.7361	NaN	3.12286	0.520482	4.89122	
220	1.16783	NaN	38.2876	21.7882	21.7885	78365.2	42.6926	-0.358012	0.355952	3.51238	NaN	NaN	-21.6327	-35	41.1457	58.2808	NaN	15.5882	0.491703	4.99524	
221	1.09862	NaN	38.2876	21.7882	21.7885	78366.2	47.224	-2.60687	0.252971	4.60245	NaN	NaN	-20.3061	-35	40.464	59.8788	NaN	12.6548	0.458448	4.49344	
222	0.296476	NaN	38.2876	21.7882	21.7885	78367.2	55.0137	-1.19289	1.01652	3.16454	NaN	NaN	-18.9796	-35	39.8149	61.5302	NaN	6.51648	0.442046	4.32043	
223	0.708825	43.9486	38.2876	21.7882	21.7885	78368.2	51.8399	0.696738	-0.645177	7.39608	-27.1542	-34.5563	-17.6531	-35	39.1999	63.2348	4.74876	11.395	0.712871	4.3039	
224	NaN	39.8024	38.2876	21.7882	21.7885	78369.2	56.0362	-4.7833	-4.03285	-0.0426168	-22.2364	-33.0117	-16.3265	-35	38.6207	64.9923	1.18171	8.9561	0.911123	4.20884	
225	0.736476	NaN	38.2876	21.7882	21.7885	78370.2	60.5039	-5.53648	0.269291	4.14157	NaN	NaN	-15	-35	38.0789	66.8014	NaN	6.29749	0.957469	4.12188	
226	0.706476	39.5866	38.2876	21.7882	21.7885	78371.2	61.7958	-3.95712	-3.94854	-0.72231	-18.7092	-34.8864	-15	-35	38.0789	66.8014	1.50775	5.00562	1.03794	4.23481	
227	1.16041	NaN	38.2876	21.7883	21.7885	78372.2	52.866	-1.15969	-2.23955	5.53459	NaN	NaN	-15	-35	38.0789	66.8014	NaN	13.9355	1.10186	4.30333	
228	1.41536	38.1256	38.2876	21.7883	21.7885	78373.2	57.2255	-5.80401	-6.46332	3.65294	-20.6387	-32.0563	-15	-35	38.0789	66.8014	0.0467	9.57591	1.41131	4.28817	
229	0.248754	37.7128	38.2876	21.7883	21.7885	78374.2	52.3167	-1.34433	-4.28569	-0.308132	-23.0537	-29.846	-15	-35	38.0789	66.8014	0.366052	14.4847	1.51772	4.48745	
230	NaN	37.3728	38.2876	21.7883	21.7885	78375.2	58.8733	-2.84755	-5.52173	-0.584534	-19.3192	-31.9921	-15	-35	38.0789	66.8014	0.706102	7.92812	1.47579	4.49755	
231	1.41092	NaN	38.2876	21.7883	21.7885	78376.2	59.8216	0.343943	-0.368405	1.68597	NaN	NaN	-15	-35	38.0789	66.8014	NaN	6.9798	1.49131	3.99738	
232	1.15648	NaN	38.2876	21.7883	21.7885	78377.2	48.1434	1.16681	-0.350529	2.29889	NaN	NaN	-15	-35	38.0789	66.8014	NaN	18.658	1.58479	4.37436	
233	1.17634	NaN	38.2876	21.7883	21.7885	78378.2	68.9197	5.04439	2.93541	6.02208	NaN	NaN	-15	-35	38.0789	66.8014	NaN	2.11826	1.7118	4.80032	
234	0.856504	37.293	38.2876	21.7883	21.7885	78379.2	53.8187	2.6405	1.62873	4.3853	-22.0156	-30.1012	-15	-35	38.0789	66.8014	0.785838	12.9827	1.58129	4.52486	
235	0.857682	37.3235	38.2876	21.7883	21.7885	78380.2	55.0083	1.56803	0.727761	3.22125	-21.4035	-30.5767	-15	-35	38.0789	66.8014	0.755351	11.7931	1.47825	4.30303	
236	0.286638	37.293	38.2876	21.7883	21.7885	78381.2	54.0447	2.35169	0.528775	3.42105	-21.8967	-30.1878	-15	-35	38.0789	66.8014	0.785838	12.7567	1.39186	4.30769	
237	0.660365	37.3165	38.2876	21.7883	21.7885	78382.2	50.2738	3.64241	2.09293	4.19953	-23.8497	-28.7004	-15	-35	38.0789	66.8014	0.762387	16.5276	1.31985	4.50716	
238	0.618397	37.3517	38.2876	21.7883	21.7885	78383.2	52	3.53046	1.83786	4.60934	-22.996	-29.4335	-15	-35	38.0789	66.8014	0.727209	14.8014	0.395282	4.63272	
239	0.863981	NaN	38.2876	21.7883	21.7885	78384.2	55.1131	2.04905	0.841254	1.67399	NaN	NaN	-15	-35	38.0789	66.8014	NaN	11.6883	0.389064	4.60643	
240	1.18125	NaN	38.2876	21.7883	21.7885	78385.2	54.0954	2.69339	1.28266	3.37409	NaN	NaN	-15	-35	38.0789	66.8014	NaN	12.7061	0.389064	4.42939	
241	1.20036	37.2367	38.2876	21.7883	21.7885	78386.2	57.2457	0.553958	-0.154573	0.315765	-20.1465	-31.316	-15	-35	38.0789	66.8014	0.842123	9.55571	0.262361	4.09908	
242	1.76403	37.2414	38.2876	21.7883	21.7885	78387.2	57.3654	1.71015	0.817682	3.18485	-20.0836	-31.362	-15	-35	38.0789	66.8014	0.837432	9.43604	0.254964	4.09362	
243	0.512825	37.3094	38.2876	21.7883	21.7885	78388.2	54.6156	2.45007	1.48176	3.9076	-21.6044	-30.4178	-15	-35	38.0789	66.8014	0.769422	12.1858	0.13601	4.06289	
244	1.69023	37.2696	38.2876	21.7883	21.7885	78389.2	56.4717	2.51809	1.9834	4.5769	-20.5858	-31.0684	-15	-35	38.0789	66.8014	0.80929	10.3297	0.043875	3.99619	
245	0.996397	37.286	38.2876	21.7883	21.7885	78390.2	56.1947	1.89873	0.82839	3.31298	-20.7449	-30.9822	-15	-35	38.0789	66.8014	0.792874	10.6067	0.0359118	3.89017	
246	0.624809	37.2672	38.2876	21.7883	21.7885	78391.2	59.1982	0.588381	-0.728141	2.36863	-19.0834	-32.0105	-15	-35	38.0789	66.8014	0.811635	7.60321	0.0348837	3.84097	
247	0.617587	NaN	38.2876	21.7883	21.7885	78392.2	50.4725	-0.0588552	-1.00308	1.31335	NaN	NaN	-15	-35	38.0789	66.8014	NaN	16.3289	0.0348837	3.57222	
248	1.11156	NaN	38.2876	21.7883	21.7885	78393.2	53.9502	1.51553	0.549166	2.25553	NaN	NaN	-15	-35	38.0789	66.8014	NaN	12.8512	0.0348837	2.48315	
249	-0.10033	37.2274	38.2876	21.7883	21.7885	78394.2	53.0565	1.10732	-0.248521	2.97052	-22.3747	-29.7532	-15	-35	38.0789	66.8014	0.851504	13.7449	0.0395836	2.50922	
250	0.797726	37.2743	38.2876	21.7883	21.7885	78395.2	56.1069	0.330839	-0.694592	2.40091	-20.7858	-30.9406	-15	-35	38.0789	66.8014	0.8046	10.6946	0.0373734	2.53764	
251	0.510254	37.279	38.2876	21.7883	21.7885	78396.2	55.4899	0.294055	-1.20924	1.88609	-21.1204	-30.7188	-15	-35	38.0789	66.8014	0.799909	11.3115	0.0370995	2.53922	
252	0.189968	37.2836	38.2876	21.7883	21.7885	78397.2	53.6706	0.594505	-0.915447	2.67438	-22.0878	-30.0366	-15	-35	38.0789	66.8014	0.795219	13.1308	0.0349625	2.24316	
253	0.881223	37.2649	38.2876	21.7883	21.7885	78398.2	59.7499	1.26625	-0.061079	3.14391	-18.7731	-32.1907	-15	-35	38.0789	66.8014	0.813981	7.05153	0.0240539	2.38978	
254	0.988271	NaN	38.2876	21.7883	21.7885	78399.2	55.9706	4.83377	3.62394	6.27867	NaN	NaN	-15	-35	38.0789	66.8014	NaN	10.8308	0.0240539	2.38961	
255	1.32148	37.0796	38.2876	21.7883	21.7885	78400.2	57.3687	-1.1459	-3.55473	4.06553	-19.9945	-31.2269	-15	-35	38.0789	66.8014	0.999249	9.43275	0.0588153	2.39411	
256	1.20012	36.294	38.2876	21.7883	21.7885	78401.2	52.7725	2.1895	0.843604	5.95895	-21.9572	-28.8987	-15	-35	38.0789	66.8014	1.78488	14.0289	0.28297	2.47765	
257	1.64769	35.5693	38.2876	21.7883	21.7885	78402.2	54.0305	-2.02676	-1.23692	4.73442	-20.8918	-28.7873	-15	-33.1579	36.3929	65.6589	0.823617	11.6284	0.283301	2.42363	
258	0.803951	34.3756	38.2876	21.7883	21.7885	78403.2	51.8125	-4.5249	-3.05727	4.51567	-21.2523	-27.0189	-15	-31.3158	34.7229	64.406	0.347258	12.5935	0.324798	2.43473	
259	0.903143	33.2312	38.2876	21.7883	21.7885	78404.2	53.9392	-1.70567	-5.92911	3.9119	-19.5613	-26.8639	-15	-29.4737	33.0711	63.0272	0.160072	9.08794	0.38435	2.49687	
260	0.868539	32.1055	38.2876	21.7883	21.7885	78405.2	56.8249	4.32153	2.26626	8.21706	-17.5681	-26.8724	-15	-27.6316	31.4405	61.5044	0.665007	4.67942	0.386795	3.0404	
261	0.872031	31.1721	38.2876	21.7883	21.7885	78406.2	46.915	0.347723	1.79949	6.97748	-21.2931	-22.7663	-15	-25.7895	29.8345	59.8163	1.33762	12.9013	0.416323	2.9231	
262	1.4314	NaN	38.2876	21.7883	21.7885	78407.2	66.2251	-11.098	-5.13492	-2.70372	NaN	NaN	-15	-23.9474	28.2573	57.9381	NaN	8.28708	0.416323	2.67199	
263	0.888698	29.9479	38.2877	21.7883	21.7885	78408.2	71.3887	-5.71478	1.40432	5.81133	-9.55778	-28.3818	-15	-22.1053	26.7141	55.8403	3.23384	15.5484	0.772355	2.89971	
264	0.578185	27.7669	38.2877	21.7883	21.7885	78409.2	53.7271	4.34046	3.68445	11.7479	-16.4278	-22.3859	-15	-20.2632	25.211	53.4889	2.55589	0.238162	0.876756	3.90741	
265	-0.123663	26.6881	38.2877	21.7883	21.7885	78410.2	51.1656	0.759945	1.96415	8.67256	-16.7354	-20.789	-15	-18.4211	23.7557	50.8446	2.93239	0.321034	0.994892	4.64277	
266	0.597254	25.9002	38.2877	21.7883	21.7885	78411.2	44.1286	1.15344	3.99689	7.76324	-18.5906	-18.0335	-15	-16.5789	22.3576	47.8624	3.54257	3.73378	1.1522	4.82901	
267	0.763912	NaN	38.2877	21.7883	21.7885	78412.2	53.5583	-8.79599	-6.77758	-0.251305	NaN	NaN	-15	-14.7368	21.0279	44.493	NaN	9.06529	1.18066	4.68656	
268	-0.23808	23.4049	38.2877	21.7883	21.7885	78413.2	45.2677	6.17545	1.80713	8.96735	-16.4722	-16.6269	-15	-12.8947	19.7807	40.684	3.62423	4.58376	1.28476	4.78809	
269	1.14648	22.7764	38.2877	21.7883	21.7885	78414.2	38.6474	8.16348	7.78481	13.2872	-17.7884	-14.2244	-15	-11.0526	18.6322	36.3844	4.14413	2.26302	1.38694	4.99227	
270	0.963143	21.9087	38.2877	21.7883	21.7885	78415.2	52.3309	1.24592	3.62421	8.49872	-13.3884	-17.3419	-15	-9.21053	17.6021	31.5514	4.30656	20.7795	1.4856	6.00018	
271	0.764708	21.2309	38.2877	21.7883	21.7885	78416.2	41.339	1.60343	1.0059	6.89049	-15.9405	-14.0233	-15	-7.36842	16.7121	26.1616	4.51882	15.1774	1.60085	6.08052	
272	1.71759	20.464	38.2878	21.7883	21.7885	78417.2	31.5818	4.84858	3.59585	8.70471	-17.4332	-10.7173	-15	-5.52632	15.9856	20.2249	4.4784	11.3569	1.60733	6.07166	
273	1.10581	19.5682	38.2878	21.7883	21.7885	78418.2	36.9364	4.56717	4.09404	9.25269	-15.6409	-11.7591	-15	-3.68421	15.4458	13.7995	4.12235	23.1369	1.47083	7.08015	
274	1.12286	18.7802	38.2878	21.7883	21.7885	78419.2	28.3482	8.25038	4.99884	10.5794	-16.528	-8.91739	-15	-1.84211	15.1127	7.00127	3.6675	21.347	1.19228	7.71896	
275	0.80342	18.1775	38.2878	21.7883	21.7885	78420.2	38.564	-0.673819	4.76453	4.16354	-14.2132	-11.3316	-15	0	15	-0	3.17748	38.564	0.892377	10.4531	
276	1.24536	17.3942	38.2878	21.7883	21.7885	78421.2	48.357	2.69782	4.4892	6.87155	-11.5582	-12.9987	-15	0	15	-0	2.39419	48.357	0.706757	13.9705	
277	-0.13908	16.7305	38.2878	21.7883	21.7885	78422.2	32.6261	7.11265	5.24268	6.59722	-14.0905	-9.02033	-15	0	15	-0	1.7305	32.6261	0.841809	14.5549	
278	0.854681	16.238	38.2878	21.7883	21.7885	78423.2	32.3111	2.34341	0.680575	10.7416	-13.7237	-8.67949	-15	0	15	-0	1.23802	32.3111	1.03071	15.1117	
279	-0.422524	15.8745	38.2878	21.7883	21.7885	78424.2	16.7042	9.15536	0.204518	10.6259	-15.2046	-4.56283	-15	0	15	-0	0.874512	16.7042	1.20875	14.3395	
280	0.877587	15.6259	38.2879	21.7883	21.7885	78425.2	20.3116	9.8242	9.40273	16.1527	-14.6543	-5.42415	-15	0	15	-0	0.625923	20.3116	1.39097	13.4093	
281	0.130087	15.443	38.2879	21.7883	21.7885	78426.2	11.7067	11.8541	8.09472	16.7122	-15.1218	-3.13341	-15	0	15	-0	0.443	11.7067	1.5419	12.8645	
282	0.582349	15.3281	38.2879	21.7883	21.7885	78427.2	5.85448	0.590027	6.58183	10.1402	-15.2481	-1.5635	-15	0	15	-0	0.328086	5.85448	1.61816	13.094	
283	0.486	15.4078	38.2879	21.7883	21.7885	78428.2	3.72762	4.3333	-2.53746	6.72301	-15.3752	-1.00171	-15	0	15	-0	0.407822	3.72762	1.69061	13.1692	
284	1.13267	15.443	38.2879	21.7883	21.7885	78429.2	6.08813	1.50651	4.29864	9.21266	-15.3559	-1.63786	-15	0	15	-0	0.443	6.08813	1.69272	12.828	
285	1.43156	15.3938	38.2879	21.7883	21.7885	78430.2	7.68404	6.59686	6.88253	9.14397	-15.2555	-2.0583	-15	0	15	-0	0.393751	7.68404	1.64298	13.249	
286	0.857448	15.4852	38.2879	21.7883	21.7885	78431.2	8.25023	10.1368	11.5101	15.2036	-15.325	-2.22207	-15	0	15	-0	0.485214	8.25023	1.51268	13.5342	
287	0.402587	15.5321	38.2879	21.7883	21.7885	78432.2	8.37649	7.48165	10.2614	13.9952	-15.3664	-2.26267	-15	0	15	-0	0.532117	8.37649	1.31686	13.6787	
288	0.636793	15.3726	38.2879	21.7883	21.7885	78433.2	8.6634	11.2338	14.5248	18.1149	-15.1972	-2.31557	-15	0	15	-0	0.372644	8.6634	1.09924	13.8753	
289	0.836754	15.2882	38.2879	21.7883	21.7885	78434.2	9.12383	10.0966	11.8555	16.0858	-15.0948	-2.42423	-15	0	15	-0	0.288218	9.12383	0.865971	14.0252	
290	0.0596505	15.2741	38.2879	21.7883	21.7885	78435.2	8.73388	7.91084	10.6623	13.4331	-15.097	-2.31931	-15	0	15	-0	0.274147	8.73388	0.611338	12.8486	
291	0.905524	15.5227	38.2879	21.7883	21.7885	78436.2	10.0696	7.36623	8.6075	13.2731	-15.2836	-2.71405	-15	0	15	-0	0.522736	10.0696	0.400228	9.0359	
292	1.10703	15.5954	38.2879	21.7883	21.7885	78437.2	9.33741	8.69737	9.99984	14.0515	-15.3888	-2.53033	-15	0	15	-0	0.595437	9.33741	0.24965	7.17302	
293	1.47203	NaN	38.2879	21.7883	21.7885	78438.2	10.1369	8.84536	10.1354	14.2525	NaN	NaN	-15	0	15	-0	NaN	10.1369	0.157554	4.13931	
294	0.467504	15.6142	38.2879	21.7883	21.7885	78439.2	10.4184	8.98131	9.95939	14.0011	-15.3568	-2.8236	-15	0	15	-0	0.614198	10.4184	0.116114	3.66533	
295	1.17314	15.5227	38.2879	21.7883	21.7885	78440.2	10.1432	9.16607	10.7297	15.0838	-15.2801	-2.73368	-15	0	15	-0	0.522736	10.1432	0.107145	2.05754	
296	0.495087	15.5157	38.2879	21.7883	21.7885	78441.2	9.79544	11.8825	13.2973	18.3296	-15.2895	-2.6397	-15	0	15	-0	0.515701	9.79544	0.108815	1.90166	
297	0.607031	15.3703	38.2879	21.7883	21.7885	78442.2	8.08834	6.07949	5.46997	11.0346	-15.2174	-2.1626	-15	0	15	-0	0.370299	8.08834	0.105727	1.76864	
298	1.27381	15.4829	38.2879	21.7883	21.7885	78443.2	7.84126	8.29654	10.198	12.6957	-15.3381	-2.11231	-15	0	15	-0	0.482869	7.84126	0.105177	1.18622	
299	0.522309	15.4219	38.2879	21.7883	21.7885	78444.2	9.15364	12.3785	13.4956	17.7806	-15.2255	-2.45335	-15	0	15	-0	0.421893	9.15364	0.10556	0.907789	
300	0.204254	15.5767	38.2879	21.7883	21.7885	78445.2	8.09022	-2.82069	-1.6931	6.27556	-15.4217	-2.19214	-15	0	15	-0	0.576676	8.09022	0.108467	0.869231	

